Adversarial Robust Memory-Based Continual Learner

Despite the remarkable advances that have been made in continual learning, the adversarial vulnerability of such methods has not been fully discussed. We delve into the adversarial robustness of memory-based continual learning algorithms and observe limited robustness improvement by directly applying adversarial training techniques. Preliminary studies reveal the twin challenges for building adversarial robust continual learners: accelerated forgetting in continual learning and gradient obfuscation in adversarial robustness. In this study, we put forward a novel adversarial robust memory-based continual learner that adjusts data logits to mitigate the forgetting of pasts caused by adversarial samples. Furthermore, we devise a gradient-based data selection mechanism to overcome the gradient obfuscation caused by limited stored data. The proposed approach can widely integrate with existing memory-based continual learning as well as adversarial training algorithms in a plug-and-play way. Extensive experiments on Split-CIFAR10/100 and Split-Tiny-ImageNet demonstrate the effectiveness of our approach, achieving up to 8.13% higher accuracy for adversarial data.

==> Figures/ATTACK.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{Images/attack.png}
  \caption{T.}
  \label{Pipeline}
\end{figure}

==> Figures/Intro.tex <==
% \begin{figure}
%   \centering
% \begin{subfigure}[t]{0.45\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{Images/Figure1_a.pdf}
% \caption{}
% \label{fig:class-il-faa}
% \end{subfigure}
% \begin{subfigure}[t]{0.45\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{Images/Figure1_b.pdf}
% \caption{}
% \label{fig:task-il-faa}
% \end{subfigure}

% \begin{subfigure}[t]{0.45\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{Images/Figure1_c.pdf}
% \caption{}
% \label{fig:class-il-forgetting}
% \end{subfigure}
% \begin{subfigure}[t]{0.45\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{Images/Figure1_d.pdf}
% \caption{}
% \label{fig:task-il-forgetting}
% \end{subfigure}

% \begin{subfigure}[t]{0.45\linewidth}
% \centering
% \includegraphics[width=1\linewidth]{Images/Figure1_e.png}
% % \caption{}
% \label{fig:caption}
% \end{subfigure}
% \caption{Il}
% %\end{subfigure}
% % \begin{subfigure}[t]{0.70\linewidth}
% % \centering
% % \includegraphics[width=1\linewidth]{Images/pipeline.pdf}
% % \caption{}
% % \end{subfigure}
% %\caption{Overview of DiReKT. The standard training model $M^{ST}$ and the adversarial training model $M^{AT}$ are trained separately. The standard training model $M^{ST}$ uses only clean samples as input, and the adversarial training model $M^{AT}$ uses adversarial samples as input. $L_{DiReKT}$ is added to keep the sample relations of the adversarial training consistent with the standard training in the feature space, thus alleviating the problem of low intra-class similarity and high inter-class similarity of the features of the adversarial training model.}
%   \label{fig:pipeline}
% \end{figure}






\newcommand\biascomparisonfigurewidth{0.47}
\newcommand\biascomparisontextwidth{0.04}

\begin{figure}
\label{fig:figure1}
\centering

\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \hspace{2pt}
    \figtext{Class Incremental}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \hspace{2pt}
    \figtext{Task Incremental}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{\hspace{16pt} FAA}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{Images/Figure1_a.pdf}
    \subcaption{}
    \label{fig:class-il-faa}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{Images/Figure1_b.pdf}
    \subcaption{}
    \label{fig:task-il-faa}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{\hspace{16pt} Forgetting}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{Images/Figure1_c.pdf}
    \subcaption{}
    \label{fig:class-il-forgetting}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \includegraphics[width=1\linewidth]{Images/Figure1_d.pdf}
    \subcaption{}
    \label{fig:task-il-forgetting}
\end{minipage}
 
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{Images/Figure1_e.png}
    \label{fig:tuli}
\end{minipage}
\caption{A preliminary analysis of the combination of continual learning and adversarial training on Split-CIFAR10 with buffer size $200$.
And we consider the final average accuracy (FAA) and forgetting of adversarial and clean samples in both class incremental and task incremental settings.
Here CL means continual learner, and ARCL means adversarial robust continual learner.
Intuitively, it can be observed that $1).$ CL is vulnerable, $2).$ ARCL enhances robustness while reducing accuracy of clean samples compared to CL, and $3).$ adversarial training accelerates forgetting of clean samples. Our method (red colour) improves FAA and forgetting for both clean and adversarial samples.} 
\label{fig:intro_old}
\end{figure}


==> Figures/Task_acc_cifar10.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{Images/task_acc_cifar10.pdf}
  \caption{Accuracy curves on the Split-CIFAR10 with buffer size $200$, and $5,120$ settings.
  The plots' x-axis denotes the total number of tasks trained cumulatively up to each learning stage. The y-axis shows the average accuracy of the current task at each respective stage.
  The results demonstrate consistent improvements across most stages of continual learning when our proposed approach is combined with the baseline model.
  }
  \label{fig:task_acc_cifar10}
\end{figure*}

==> Sections/5_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
In this paper, we design algorithms to improve adversarial robustness for memory-based continual methods, and in the future we plan to investigate how to improve adversarial robustness of other types of continual learning algorithms, such as dynamic architecture or regularization-based continual methods.
What's more, our proposed AFLC not only works for adversarial robust continual learning but also standard continual learning. More related details can find in Appendix.
% \input{Tables/Ablation2}


==> Sections/7_bak.tex <==
\section{Baselines and their inherent problems}
\label{sec:analysis}
In this section, we first give a brief formulation of memory-based continual learning and adversarial training framework.
Then we systematically examine some of the popular memory-based continual learning algorithms and explore their combination with adversarial training.
We throw further light on new problems under adversarial robust continual learning and analyze the underlying causes, which motivate us to develop our approach in Section~\ref{sec:method}.
\input{Tables/Analysis}
\subsection{Preliminaries}

\paragraph{Memory-based Continual Learning}
We consider the scenario of continual learning $T$ classification tasks.
The data distribution for the $t$-th task ($1 \le t \le T$) is $D_t$, $x$ is the input sample and $y$ is the label.
% The dataset for the $t$-th task ($1 \le t \le T$) is $D_t = \langle x_t, y_t \rangle$, where $x_t$ is the input data and $y_t$ is the label.
% Taking the classification task as an example, formally a continual learning problem is divided into $T$ tasks; in each task $t \in \{1, ... , T\}$, the input data $x_t$ of task $t$ with their respective labels $y_t$ are sampled from an i.i.d. distribution $D_t$.
A function $f(\cdot)$ with parameters $\theta$ is optimized sequentially in the given task order.
We denote the output logits as $h_{\theta}(x) \in \mathbb{R}^{C}$, where $C$ is total number of categories, and the probability distribution $f_{\theta}(x)=\mathrm{softmax}(h_{\theta}(x))$.
The goal of continual learner is to correctly classify data of all observed tasks, and its objective can be formalized as:
\begin{equation}
    \begin{aligned}{
\mathop{\arg\min}_{\theta} \sum_{t=1}^{T}  \mathcal{L}_{t}, \ \ \mathrm{where} \ \  \mathcal{L}_{t} \triangleq \mathbb{E}_{(x,y)\sim D_t}[ \ell (y,f_{\theta}(x))],}
    \end{aligned}
\end{equation}
where $\ell$ is the task-specific loss, and $t_c$ denotes the current task.
The unavailability of past task data poses great challenges to continual learning, as direct sequential optimization results in severe catastrophic forgetting.
% in terms of optimization, which results in catastrophic forgetting.

Face to the above challenge, memory-based continual learners invariably outdo leading-edge approaches by storing a few past task data and replaying them during the current task training phase~\cite{buzzega2020dark,9891836}.
% Memory-based continual learner tries to store a few past task data and replay them during the current task training phase to alleviate this problem, which is by far the most effective way.
When training the $t$-th task, its loss function can be formalized as the following:
\begin{equation}
\begin{aligned}
\ell (y_{t},f_{\theta}(x_t)) + \ell(y_{\mathcal{M}},f_{\theta}(x_{\mathcal{M}})), 
\end{aligned}
\end{equation}
where $\mathcal{M}$ is the episodic memory of the current task, which preserves a small subset of observed data $\langle x_{\mathcal{M}},y_{\mathcal{M}} \rangle$ of past tasks.

\paragraph{Adversarial Training}
Adversarial training is currently the most reliable way~\cite{bai2021recent} to improve the adversarial robustness of a model.
Following~\cite{madry2018towards}, it can be formally defined as a min-max optimization problem:
\begin{equation}
\mathop{\arg\min}_{\theta} \mathbb{E}_{(x, y) \in D}\left(\max_{\delta \in S} { \ell}(f_{\theta}(x+\delta), y)\right),
\label{eq:at}
\end{equation}
where $\delta$ is an adversarial perturbation, $D$ is data distribution, and $S$ is a perturbation set.
$S =\left \{ \delta | \left \| \delta \right \|_{p} \le \epsilon  \right \}$, $\epsilon$ is the perturbation size. The goal of adversarial training is to correctly classify all adversarial examples ($\widetilde{x} = x+\delta$).

Here we integrate memory-based continual learner and adversarial training as adversarial robust memory-based continual learner baselines, and the new optimization objective during the training stage of $t$-th task is:
\begin{equation}
\mathop{\arg\min}_{\theta} \mathbb{E}_{(x, y) \in D_{t} \cup M}\left(\max_{\delta \in S} { \ell}(f_{\theta}(x+\delta), y)\right).
\label{eq:total}
\end{equation}




\subsection{Performance of the baselines}

We present a detailed and systematic analysis starting from popular memory-based continual learning methods: ER~\cite{riemer2019learning}, DER/DER++~\cite{buzzega2020dark} and ER-ACE~\cite{caccia2022new} with different memory buffer sizes on the Split-CIFAR10~\cite{krizhevsky2009learning} dataset.
As shown in Table \ref{Analysis}

We implement these methods with both standard and adversarial training and test them with clean and adversarial data.
Following~\cite{buzzega2020dark}, we consider class incremental and task incremental two different settings, and our evaluation metrics are final average accuracy (FAA) and forgetting in the scenarios of both clean data and under attack for each continual learning method.


We also design clean relative decrease (CRD), which measures clean FAA performance degradation before and after adding adversarial training;
forgetting relative increase (FRI), which measures clean forgetting elevation before and after adding adversarial training;
and robust relative decrease versus joint model (RRD), which measures the gap in robustness improvement due to adversarial training compared to the joint model, three special metrics to better analyze the changes in the continual learners before and after combining the adversarial training.
More metric details on Appendix.
% We observe their performance under adversarial attacks and combine them with adversarial training to compute their Final Average Accuracy(FAA) and Forgetting for clean and adversarial samples respectively, in order to investigate the impact of adversarial training on the continual learning model in terms of natural generalization, robustness generalization and forgetting.
% Here we use PGD-20 with $\epsilon = 8/255$ to generate adversarial examples.
% And our findings can be summarized below.

Firstly, larger scale experiments have further validated the observations of Sec.~\ref{sec:intro}.
Standard continual learners are vulnerable; combined with adversarial training, continual learning models improve robustness while reducing clean performance (CRDs are all positive); and adversarial training accelerates the forgetting of clean samples (FRIs of memory-based CLs are all positive), while robustness also forgets.

What's more, \textbf{growth in buffer size leads to an overall improvement in performance}.
By comparing the M-ARCL results for different buffer sizes, we find when buffer size is $5210$, the model has significant improvements both on clean/adversarial FAA/forgetting metrics compared to $200$ buffer sizes, adversarial FAA is in class incremental settings (class-il) are up to $14.12\%$ and $17.44\%$ for task increment settings (task-il); adversarial forgetting can be reduced up to $27.92\%$ on class-il and $17.69\%$ on task-il.
The improvement on clean data of class-il is more obvious. The FAA can be improved by up to $33.70\%$, the forgetting can be relieved by up to $42.87\%$, the task-il FAA can be improved by $8.66\%$ while forgetting relieved by $9.63\%$.

Finally, Table~\ref{Analysis} demonstrates that \textbf{adversarial training is not suitable for direct integration with continual learning models}.
Initially, we notice that for the same amount of data and super-parameters, the improvement in robustness of the continual learning model with adversarial training is quite inferior to that of the joint model (RRDs are all positive).
Meanwhile, when DER/DER++ and ER-ACE are combined with adversarial training, they show favourable stability in the stability-plasticity dilemma, disproportionately inhibiting learning ability on the new task.
In contrast, the combination of ER and vanilla AT show superior robustness performance in the analysis experiments, and we therefore use ER as a basis for exploring our approach and comparing it with other adversarial training algorithms.
% big buffer size is all you need
% \paragraph{The influence of buffer size}
% As more data is stored, we find that the model improves FAA for both clean and adversarial samples, both class-il and task-il , while catastrophic forgetting is also mitigated
% And the larger the memory buffer size, the more robust and less forgetful they are.
% Meanwhile, More advanced work such as ER-ACE, DER, and DER++, perform worse in terms of robustness compared to the classical algorithm ER.
% 直接结合对抗训练和持续学习是不合适的
% \paragraph{ddd}
% There is catastrophic forgetting in robustness, and increasing the buffer size can effectively mitigate robust forgetting.
% What's more, we note a further problem specific to robust continual learning: adversarial training accelerates the forgetting of continual learners on clean samples. We will explore this issue in more detail in the next sub-section.
% The learning capacity required to achieve robustness is~cite{} greater than for the common task.
% However, when DER/DER++ and ER-ACE are combined with adversarial training, they show favourable stability in the stability-plasticity dilemma, disproportionately inhibiting learning ability on the new task.
% In contrast, the combination of ER and vanilla AT show superior robustness performance in the analysis experiments, and we therefore use ER as a basis for exploring our approach and comparing it with other adversarial training algorithms.

\subsection{The inherent problems}
A deeper analysis of the above phenomena is carried out to design better robust continual learning models, and two problems inherent in the direct combination of adversarial training and continual learning are identified.


\paragraph{CL to AT: Gradient Obfuscation}
% We observe particular gradient obfuscations in adversarial training under continual learning.
We observe a new particular type of gradient obfuscation in adversarial training under continual settings, which results in minor robustness improvements compared to the joint model.
% Badly, there is continual-specific gradient obfuscation during adversarial training.
Gradient obfuscation~\cite{athalye2018obfuscated} is caused by non-differentiable operators, unstable values, randomness in the testing phase or deep computing.
Unlike the previous causes, gradient obfuscation under continual learning is due to limited replay data.
% We identify three types of obfuscated gradients: shattered gradients are nonexistent or incorrect gradients caused either intentionally through non-differentiable operations or unintentionally through numerical instability; stochastic gradients depend on test-time randomness; and
% vanishing/exploding gradients in very deep computation result in an unusable gradient.
When constructing class boundaries for the old and new tasks, the model has only a small number of old task samples, which result in overfitting to the data in memory and direction-biased gradients when generating adversarial examples.
As shown in Figure~\ref{fig:gradient_similarity}, we calculate the gradient directions of the adversarial robust joint model and continual model, and we find that there is a significant difference between the gradient directions of the continual learner and the joint learner, which leads to lower adversarial robustness for continual learners.
% comparing the continual learner and the joint learner combined with adversarial training, we find that the adversarial samples generated by the joint learner can easily attack the continual learner, but not the other way round; in addition, we compare the gradient directions of the two, and we find that there is a significant difference between the gradient directions of the continual learner and the joint learner.
% This is one of the reasons for the low class incremental robustness for continual learners.
\paragraph{AT to CL: Accelerated Forgetting}
% \paragraph{AT for CL: Greater Negative Gradients Against Past Tasks}
As mentioned above, adversarial training accelerates the forgetting of continual learners on clean data.
This is due to the properties of the adversarial sample.
We set $h_{\theta}(x) = [h_{\theta}(x)_{1}, ..., h_{\theta}(x)_{i}, ..., h_{\theta}(x)_{C}]$, where $h_{\theta}(x)_{i}$ means the logit corresponding to the $i$-th class of sample $x$.
We can divide $h_{\theta}(x)$ into three parts: $h_{\theta}(x)_{p}$, $h_{\theta}(x)_{c}$, and $h_{\theta}(x)_{f}$.
$h_{\theta}(x)_{p}$ means the logits of past classes of $x$, $h_{\theta}(x)_{c}$ means the logits of current classes of $x$, and $h_{\theta}(x)_{f}$ means the logits of future classes of $x$.
According to~\cite{madry2018towards}, 
\begin{equation}
\begin{aligned}
\widetilde{x} = x+\delta, \ \ {\rm where} \ \delta \triangleq \arg\max_{\delta \in S} { \ell}(f_{\theta}(x+\delta), y),
\end{aligned}
\end{equation}
adversarial sample raises the logit corresponding to the other categories, and data from current task $t$ are vulnerable data prone to attack as past categories especially in the early training stages.
It can be naturally implied that the adversarial sample $\widetilde{x_{t}}$ of current task has a higher logit in the other categories compared to the clean sample $x_{t}$, while its own true category corresponds to a lower logit.
Namely,
\begin{equation}
\begin{aligned}
h_{\theta}(\widetilde{x_{t}})_p > h_{\theta}(x_{t})_p, \ h_{\theta}(\widetilde{x_{t}})_{c} < h_{\theta}(x_{t})_{c},
\end{aligned}
\end{equation}
which results in greater negative gradients towards the past tasks, especially in the early training stages of the new task.
% \input{Figures/ATTACK}
\input{Figures/GRADIENT}

% Figure~\ref{} supports our view that the norm of the adversarial samples gradient in the training phase is significantly higher than that of the clean samples, and the negative gradient of the new task adversarial samples to the earlier task classifier parameters is higher than the clean samples at the time of the training task switch.

==> Sections/_BAK_0_abstract.tex <==
\begin{abstract}
   Continuous learning has recently attracted the attention of an increasing number of researchers.
   However, existing works have not yet focused on the security risks of continual learners under adversarial attacks.
   In this work, we explore the adversarial vulnerability of continual learning and how to construct adversarial robust continual learners.
   Specifically, we have made a systematic study of existing meomory-based continual learning methods with adversarial training frameworks.
%   We first reveal that a simple combination of both leads to forgetting acceleration and gradient obfuscation.
%   Then we propose a new memory-based adversarial continual learner.
We find that directly equipping memory-based methods with adversarial training exacerbates catashtrophic forgetting, a reflection of the gradient obfuscation phenomenon.
Motiviated by this, we propose a new memory-based adversarial continual learner.
we propose to calibrate the logit of past and present tasks for weakening of negative gradients to past tasks.
We further devise data selection mechanisms based on robust difficulty to alleviate robust forgetting.
Extensive experiments have demonstrated the effectiveness of our approach.
Our method is also applicable to different memory-based continual learning methods.
% Extensive experiments demonstrate the superiority of our approach over other state-of-the-art defense methods. To the best of our knowledge, we are the first work to formulate the problem of adversarial robust continual learning. We believe that this will be an important step towards real-world continual learning.
\end{abstract}

==> Sections/_BAK_1_introduction.tex <==
% Introduction的主要问题（2022.10.23）by yzh：
% 1. 读起来不像introduction。Introduction的目的是论述工作的重要性：每一段需要很好的衔接，让人连着读下去；读完之后就应该让人十分认可，愿意接着向下读（或功利地说，让人有接收的欲望）。
%
% Introduction大概的逻辑应该是：文章所在的领域很重要 - 领域内很多重要工作 - 这些工作都没有解决领域内仍存在的一个重要挑战（在此提出文章欲解决的科研问题）- 存在几个和这个挑战非常相关的工作 - 但他们都存在这样那样的问题，没能完全解决这个挑战（这里再次强调这个挑战真的很重要而且没人(正面)做过）- 我们是怎么做的（提出了XX框架 - 采用YY做法 - 得到ZZ效果，效果很出色）。
% 就像推手一样，不断的“抛出论述（前人工作） - 反驳前人工作（哪里做的不够好）”过程串联起紧凑的逻辑，环环相扣让人挪不开视线。
%
% Introduction应该像诸葛亮在阵前的发言一样，是high-level的“以理服人”，极少见在introduction部分就说做了什么实验，甚至报告实验结果和分析的。目前的introduction部分的主要问题就是读起来像一个实验报告。第二段就说"conducted a systematic analysis"，后面还跟着分析；第三段、第四段又是两个更深入的分析，这些完全可以放在实验部分的前几节，相对不重要的可以放在discussion甚至appendix里。
%
% 根据本工作的具体情况，我建议introduction部分分成以下几段：
% ① 深度学习获得成功，但仍存在两个问题：a. 输入微小扰动就可能导致模型给出完全不同的输出；b. 无法在流式任务下进行持续学习。这两个问题均限制了深度学习在现实场景中的应用。
% ② 现有工作分别address这两个问题：有若干工作致力于持续学习，但都不鲁棒。有若干工作致力于对抗防御，但大都针对经典的单任务学习场景，未考虑持续学习场景。我们提出问题：能否获得对抗鲁棒的持续学习者（continual learner）？
% ③ 与我们相近的研究方向有order-robust continual learning，但他们关注的是任务顺序的鲁棒性，没有考虑输入扰动情形下的鲁棒性。唯一/唯二/..的几个工作部分回应了我们的问题（怎么做的blablabla），但仍存在问题（通过与我们工作最特殊的贡献进行比较，概括他们所没做到的地方，写在这里）。因此如何获得对抗鲁棒的持续学习者（continual learner）仍然是一个难题。
% ④ 我们的方法。在这一工作中，我们关注memory-based持续学习算法，提出XXX框架。。大致做法。。取得怎样的结果。
%
% 关于直接结合对抗训练的做法以及其存在的问题（加剧forgetting, gradient obfuscation等），都属于具体实验分析的一部分了，可以放到后面section再说。Contributions的罗列，以及篇章结构的组织，视版面空余情况可说可不说。在第一页右上角放上精致的方法示意图。

% 2. Introduction的每一句论述都需要有论据支撑。如第一句说“深度学习有很多实际应用”就需要跟上许多引用，如计算机视觉、自然语言处理、机器人学等应用的经典工作。修改时需要注意在类似的“主观”论述后面加上引用。

% 3. 文字还比较青涩，存在一些语法错误，后期修改时应注意完善。

% 附上孙茂松老师关于introduction写作的口诀，可以参考（摘自孙老师的微博）：
% 主题扣标题，议题扣主题。逻辑定层次，层次定语次。一事两三句，长处到短处。一理两三句，短处到长处。事理环环扣，奔向创新处。

% Introduction的主要问题（2022.11.5）by yzh：注意语法问题，另外偶尔有偏主观的表述要避免；再refine一些后可请老师和同学审读一下，让大家指出主观/青涩的地方

\section{Introduction}
\label{sec:intro}
% 按照宗瀚UU的建议改的新版本

Deep neural networks are widely used in various real-life worlds, such as self-driving~\cite{badue2021self}, face recognition~\cite{kortli2020face,meng2021magface,du2022elements}, object tracking and detection~\cite{meinhardt2022trackformer,pang2022zoom}, and more.
However, deep models usually are vulnerable to adversarial examples~\cite{szegedy2013intriguing,duan2021advdrop,zhang2022towards,10132429}, and problematic when dealing with streaming non-\textit{i.i.d.} data, which brings catastrophic forgetting~\cite{mccloskey1989catastrophic,ratcliff1990connectionist}.
Both of these limitations restrict the further application of deep learning in real-world scenarios.

A great deal of work looks to challenge both of these barriers.
Many researchers~\cite{parisi2019continual} devote to improving the continual learning capability of the model, which is currently divided into memory-based~\cite{riemer2019learning,buzzega2020dark,caccia2022new}, regularization-based~\cite{kirkpatrick2017overcoming,li2017learning,lin2022towards}, and dynamic architecture~\cite{rusu2016progressive,wang2022learning,douillard2022dytox}.
Yet none of them take into account the threat of adversarial attacks.
\cite{akhtar2018threat,bai2021recent} attempt at adversarial robustness strengthening of the model, and adversarial training has shown to be the strongest defence available~\cite{madry2018towards,zhang2019theoretically,maini2020adversarial,pang2021bag,croce2021robustbench,cui2021learnable,pang2022robustness}.
But mostly only for single-task learning scenarios.
continual learning does not have access to data from past tasks while adversarial robustness generalization has more data requirements~\cite{schmidt2018adversarially}.
Therefore, it remains a challenge to achieve adversarial robustness and continual learning simultaneously.
% which means that achieving robustness and continuation at the same time is a very ambitious problem.
% So, how can we get a adversarial robust continual learner?

Some work has also considered the robustness of continual learning models.
\cite{farquhar2018towards,yoon2019scalable,wu2021pretrained} puts emphasis on the impact of different experimental settings, on the performance of continual learners, such as task order, time/compute/memory constraints, architectures, and more; and ignores potential safety vulnerabilities.
\cite{umer2020targeted} has also focused on the security risks to continual learners, but they have focused on the risks posed by backdoor attacks during the training phase, and \cite{hassanpour2022differential} pays attention to privacy preservation, and they all ignore the threat of adversarial attacks during the testing phase.
Therefore it is still a challenge to obtain an adversarial robustness continual learners.

% ④ 我们的方法。在这一工作中，我们关注memory-based持续学习算法，提出XXX框架。。大致做法。。取得怎样的结果。
%问题难点：1、持续学习的难点在无法获取旧任务数据，而鲁棒性对数据的需求量比自然泛化性要求更高；
% 2.持续学习的挑战在于stability-plasticity dilemma，而目前有工作认为鲁棒性需要模型更强的学习能力，这意味着之前的持续学习工作找到的平衡并不适用于鲁棒持续学习；
% 3.持续学习目前最大的问题是灾难性遗忘，而对抗训练会造成干净样本准确率下降
% The core problem of continual learning is catastrophic forgetting~\cite{}, and storing a small number of past task data and replaying are the most promising direction to mitigate that.
% The challenge of continual learning is to prevent catastrophic forgetting, while adversarial training reduces the generalizability of clean samples and tends to over-fit to the training set, which means that a direct combination of the two faces significant challenges.
In this work, we focus on memory-based continual learning algorithms and adversarial training because of their superior performance.
Through experimental analysis, we find that standard memory-based continual models without adversarial defenses are all very vulnerable.
And continual learning model combined with adversarial training exacerbates the catastrophic forgetting of natural samples because that negative effects of adversarial data on past task parameters are significantly higher than that of clean samples, especially in the early stage of task switching.
What's more, compared with the joint model, the continual model can only rely on a small number of samples to establish robust boundaries between tasks, which leads to gradient obfuscation.

To mitigate the aggravation of catastrophic forgetting, we propose Anti-Forgettable Logit Calibration (AFLC).
We rectify the data in the logit layer by subtracting a larger prior from the logit position corresponding to the past class, expanding the margin between the past class and the current class, and thus attenuating the negative gradient of the adversarial sample of the new data to the past task.
In addition, to reduce robust forgetting, we propose Robustness-Aware Experience Replay (RAER) by selecting data according to the robust difficulty factor $K$.
Our approach can be combined with most continual learning as well as adversarial training algorithms, and we have demonstrated the effectiveness of our approach on the CIFAR-10 and CIFAR-100 datasets.
% Most deep learning algorithms are under classical settings, however, the model usually can not access past task data during learning the current task in real-life scenarios.
% Therefore, continual learning has attracted the attention of many researchers.
% % At present, the direction of continual learning~\cite{} mainly focuses on three directions: memory-based~\cite{}, regularization-based~\cite{}, and  architecture-based~\cite{}, among which the effect of memory-based Continual Learning Methods is far ahead.
% What's more, deep learning models are vulnerable to adversarial examples~\cite{}.
% However, adversarial robustness in continual learning is still an largely unexplored problem.
% % In order to enhance the adversarial robustness of the model, many works of adversarial defense~\cite{} have been proposed.In addition to ideal datasets, there is also a lot of research on model adversarial robustness in the more real-world setting of long tail~\cite{}, open set~\cite{} and more.
% %第二段写持续学习和对抗训练的经典问题，同时他们俩的组合会产生新的问题
% %刚改完第一段，剩下的明天再改吧....
% % 新Baseline跑上了,继续改！

% To shed light on the challenges of adversarial robustness under continual learning, we conducted a systematic experimental analysis.
% Adversarial training has been proven the most effective methods to improve adversarial robustness.
% However, adversarial training shows obviously natural test accuracy decay and catastrophic overfitting~\cite{}.
% Meanwhile, the core problem of continual learning is catastrophic forgetting~\cite{}, and storing a small number of past task data and replaying are the most promising direction to mitigate that.
% After experimental testing, we find that memory-based continual models that are not hardened by adversarial defenses are all very vulnerable, and the continual learning model combined with adversarial training exacerbates the catastrophic forgetting of natural samples, and shows gradient obfuscation during training.
% % So, combining adversarial training and continual learning directly will accelerate forgetting and enhance overfittings on memory data.


% % To sheld light on the challenges of adversarial robustness under continual learning, we conducted a systematic experimental analysis.
% % The systematic research is carried out under two Settings: class incremental and task incremental. 
% % We find that memory-based continual models that are not hardened by adversarial defenses are all very vulnerable.
% % To improve the robustness of continual model, it is natural to combine with adversarial training,  the most effective adversarial defense method.  
% % It is found that after adversarial training, the continual learning model exacerbates the catastrophic forgetting of clean samples, and gradient obfuscation occurs during training.
% %第三段介绍新问题的深入分析:先是为什么遗忘会加剧
% % We further explore why adversarial training makes the forgetting worse.
% On the one hand, through theoretical and empirical analysis, we find that the negative effect of adversarial samples on past task parameters is significantly higher than that of clean samples especially in the early stage of task switching.
% As show in Figure~\ref{fig:onecol}, adversarial data have higher soft-max margins between past tasks and current tasks, and bigger gradient norm gaps between buffer data and current data, which result in larger gradients to past task parameters.
% Since adversarial samples are obtained from natural samples along the direction of gradient ascent, and samples can be easily attacked as the category of past tasks when the new task just start training, this larger negative gradient from adversarial examples to past tasks will lead to the acceleration of forgetting.
% % 然后再解释梯度混淆

% On the other hand, compared with the joint model, the continual model can only rely on a small number of samples to establish robust boundaries between tasks, which leads to gradient obfuscation.
% As show in Figure~\ref{fig:onecol}, continual model shows low defense accuracy under the adversarial examples generated by joint model, and few gradient similarity with joint model for the same data.

% 我们的做法
% To mitigate the aggravation of catastrophic forgetting, we propose adaptive logit adjustment for adversarial robust continual learning.
% \cite{} add logit masks to the new task to avoid affectness of classifier parameters of the past task, but these methods ignore that the feature extractor is common, and the old task will still be affected by the gradient of the new task. 
% The characteristics of adversarial samples make the forgetting performance of feature extractor more obvious.

% In addition, in order to better improve the robustness of the model, we selected data according to the robustness.
% the model only accesses a few past data, great number of current data and none of future data due to specific settings of continual learning.
% Compared with the joint model, the continual model can only rely on a small number of samples to establish robust boundaries between tasks, which leads to gradient obfuscation.
% We experimentally find that when switching between the old and new tasks, compared with the clean samples, the data distribution of the adversarial samples of the new task in logit space overlaps more obviously with that of the old task. Let now be the TTH task. A lot of new task data $D_ {t} = \{X_ {t}, Y_ {t} \} $generated against sample $X ^ {adv} _ {t} $, it into the model output respectively $logit_ {t}, logit ^ {adv} _ {t} $, cite mentioned, when the old and the new task switching, The logit[: t] value of the data of the new task corresponding to the old task class will be larger than the real class logit[t] value, and the adversarial samples will increase this GAP. Therefore, when calculating the gradient, the adversarial samples will have a greater negative impact on the parameters corresponding to the old task. Similarly, for the samples in Buffer, the gradient generated when updating the model with adversarial examples is larger, resulting in the model easier to Overfitting to the small number of samples stored. This further leads to more significant overlapping of the data distribution between different tasks in logit space for adversarial trained models. ** One more experiment is needed here, The Logit space of the final model that is verified by adversarial training will have more overlapping (just calculate the KL distribution directly)**, which leads to the forgetting of model robustness and the forgetting of clean generalization. In addition, due to the special experimental setting of continual learning, the model can only see a small amount of past task data and a large amount of current task data during training, and cannot obtain future task data, which leads to the gradient of the model mainly concentrated between the boundaries of current task data, resulting in **gradient obfuscation**.

% For **gradient obfuscation**, we believe that the training process should not trust the gradient too much, pursue "strong adversarial examples", and adopt friendly AT to alleviate the dependence on strong adversarial examples. To mitigate the ** catastrophic forgetting of clean samples **, we also [cite] a logit mask. For the negative gradient of the old task when the new task is updated, [cite] chooses to add logit mask to the new task to avoid affecting the parameters of the old task classifier, but these methods ignore that the feature extractor is common, and the old task will still be affected by the gradient of the new task. The characteristics of adversarial samples make the forgetting performance of feature extractor more obvious after adversarial training. To further improve the robustness and clean generalization of catastrophic forgetting, we comprehensively consider the difficulty of adversarial examples, the order of task learning, the number of samples of different categories, adaptive logit adjustment for adversarial robust continual learning is designed. When doing adversarial training at the same time, different intensity of confrontation is required for the new task and the old task. Experiments demonstrate the effectiveness of our method.

Our contributions can be summarized in the following three points:
\begin{itemize}
	\item As far as we know, we are the first work to study adversarial robustness under continual learning setting.
We believe this is an important step towards realistic continual learning.
	\item We systematically analyze the existing memory-based continual learning algorithms and their performance in combination with adversarial training, and find two problems under this new scenario: adversarial training will accelerate the forgetting of the continual learning model, and the gradient obfuscation in the continual learning scenario.
	\item We propose a simple but effective algorithm to improve the adversarial robustness of continual learners , which can effectively alleviate the above two problems.
\end{itemize}

==> Tables/Ablation1_std.tex <==
\begin{table*}[]
    \centering % 居中显示
        \caption{Ablation experiments on the Split-CIFAR10 dataset with the buffer size of $200$, using ER+TRADES as the baseline.  \textbf{Bold} indicates that the inclusion of this module will relatively enhance the corresponding evaluation metrics. Experiments have demonstrated that AFLC mitigates clean-sample accelerated forgetting from adversarial samples, RAER mitigates gradient obfuscation (Adversarial FAA has a boost) and robust forgetting; adding FP improves the model's ability to learn new tasks (FAA has an overall increase).}
    \label{Ablation1_std}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lllll lll lll}
    \toprule
    \multirow{3}{*}{\textbf{AFLC}} &
    \multirow{3}{*}{\textbf{RAER}}&
    \multirow{3}{*}{\textbf{FP}}&
    \multicolumn{4}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{4}{c}{\textbf{Task Incremental Setting}} \\
    ~&~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{2}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{2}{c}{\textbf{Adversarial Data}}\\
    ~&~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&\textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&\textbf{Forgetting$\downarrow$}\\
    \midrule
    & & &$22.42_{\pm{7.11}}$& $77.25_{\pm{10.79}}$& $15.72_{\pm{0.82}}$& $64.95_{\pm{5.58}}$& $78.79_{\pm{0.81}}$& $8.1_{\pm{0.97}}$& $51.33_{\pm{2.3}}$& $21.97_{\pm{1.31}}$ \\
    % $\usym{2713}$& & & \pmb{$38.85_{\pm{3.26}}$}& \pmb{$47.53_{\pm{21.21}}$}& \pmb{$17.56_{\pm{1.4}}$}& \pmb{$42.80_{\pm{21.82}}$}& \pmb{$82.70_{\pm{0.43}}$}& $9.97_{\pm{1.04}}$& $50.67_{\pm{6.55}}$& $26.28_{\pm{10.45}}$ \\
    $\usym{2713}$ & & & $37.88_{\pm{0.54}}$& $21.76_{\pm{0.23}}$& $18.58_{\pm{1.9}}$& $21.77_{\pm{0.24}}$& $81.66_{\pm{0.02}}$& $10.86_{\pm{0.78}}$& $53.64_{\pm{1.48}}$& $17.6_{\pm{0.28}}$\\
   
    $\usym{2713}$&$\usym{2713}$& &$37.45_{\pm{5.28}}$& \pmb{$10.29_{\pm{11.36}}$}& \pmb{$19.81_{\pm{1.75}}$}& \pmb{$9.61_{\pm{6.38}}$}& $78.13_{\pm{3.1}}$& $15.39_{\pm{4.28}}$& \pmb{$55.71_{\pm{3.47}}$}& \pmb{$14.13_{\pm{3.09}}$} \\
    $\usym{2713}$&$\usym{2713}$&$\usym{2713}$& \pmb{$43.34_{\pm{4.27}}$}& $33.40_{\pm{11.02}}$& \pmb{$19.85_{\pm{1.55}}$}& $30.78_{\pm{8.84}}$& \pmb{$82.59_{\pm{1.12}}$}& \pmb{$7.53_{\pm{1.24}}$}& \pmb{$59.41_{\pm{0.61}}$}& $14.16_{\pm{1.29}}$  \\
\bottomrule
\end{tabular}}

\end{table*}

==> Tables/Ablation2_std.tex <==
% \begin{table*}[]
%     \caption{Data selection strategy ablation experiments on the CIFAR-10 dataset with the buffer size of 200, using ER + Vanilla AT as the baseline.
%     When $\rho = 11$, this is equivalent to not applying the robust data selection strategy.}
%     \label{Ablation2}
%     \centering % 居中显示
%     \scalebox{1.0}{
%     \begin{tabular}{lll lll lll}
%     \toprule
%     \multirow{3}{*}{\textbf{$\rho$}} &
%     \multicolumn{4}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{4}{c}{\textbf{Task Incremental Setting}} \\
%     ~&\multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{2}{c}{\textbf{Adversarial Data}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{2}{c}{\textbf{Adversarial Data}}\\
%     ~&\textbf{FAA }&\textbf{Forgetting}&
%     \textbf{FAA}&
%     \textbf{Forgetting}&
%     \textbf{FAA }&\textbf{Forgetting}&
%     \textbf{FAA }&\textbf{Forgetting}\\
%     \midrule
%     \textbf{$11$}& $28.18$ & $80.58$ & $17.86$ & $69.58$ & $84.49$ & $10.23$& $44.30$ & $36.89_{\pm{1.11}}$  \\
%     \textbf{$8$}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 \\
%     \textbf{$5$}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0  \\
%     \textbf{$2$}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 \\
% \bottomrule
% \end{tabular}}
% \end{table*}


% \begin{table*}[]
    
%     \centering % 居中显示
%     \scalebox{0.7}{
%     \begin{tabular}{lll ll}
%     \toprule
%     \multirow{2}{*}{\textbf{$\rho$}} &
%     \multicolumn{2}{c}{\textbf{Class-IL}} &
%     \multicolumn{2}{c}{\textbf{Task-IL}} \\
%     ~&{\textbf{Clean FAA}}&
%     {\textbf{Adversarial FAA}}&
%     {\textbf{Clean FAA}}&
%     {\textbf{Adversarial FAA}}\\
%     \midrule
%     \textbf{$11$}& \pmb{$28.18$} & $17.86$ & $84.49$& $44.30$ \\
%     \textbf{$8$}&$27.66$ &$17.80$ & $86.28$ & $46.15$  \\
%     \textbf{$5$}&$27.60$ & \pmb{$18.00$}& \pmb{$86.20$} & \pmb{$48.45$}   \\
%     \textbf{$2$}&$27.06$ & $17.83$ & $85.97$ &$47.93$ \\
%     \midrule
%     \textbf{$k \geq 5$}&$20.49$ & $15.74$ & $72.94$ &$31.15$ \\
% \bottomrule
% \end{tabular}}
% \caption{Data selection strategy ablation experiments on the CIFAR-10 dataset with the buffer size of 200, using ER + TRADES as the baseline.
%     When $\rho = 11$, this is equivalent to not applying the robust data selection strategy.}
%     \label{Ablation2}
% \end{table*}


% \begin{table*}[]
    
% \centering % 居中显示
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lllllllll}
%     \toprule
%     \multirow{3}{*}{\textbf{$\rho$}}&
%     \multicolumn{4}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{4}{c}{\textbf{Task Incremental Setting}} \\
%     ~&\multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{2}{c}{\textbf{Adversarial Data}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{2}{c}{\textbf{Adversarial Data}}\\
%     ~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{FAA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}\\
%     \midrule
%     \textbf{$11$}&$22.42_{\pm{7.11}}$& $77.25_{\pm{10.79}}$& $15.72_{\pm{0.82}}$& $64.95_{\pm{5.58}}$& $78.79_{\pm{0.81}}$& $8.10_{\pm{0.97}}$& $51.33_{\pm{2.3}}$& $21.97_{\pm{1.31}}$ \\
%     % \textbf{$11$}& $18.32_{\pm{0.47}}$& $83.37_{\pm{2.82}}$& $15.30_{\pm{0.5}}$& $68.17_{\pm{0.08}}$& $78.97_{\pm{1.06}}$& $7.74_{\pm{1.05}}$& $52.64_{\pm{0.67}}$& $21.81_{\pm{1.82}}$\\
%     \textbf{$10$}& $18.04_{\pm{0.58}}$& $84.61_{\pm{1.98}}$& $15.31_{\pm{0.18}}$& $68.33_{\pm{2.31}}$& $80.38_{\pm{0.16}}$& $7.06_{\pm{0.93}}$& $59.88_{\pm{1.21}}$& $13.78_{\pm{0.97}}$ \\
%     \textbf{$5$}& $18.21_{\pm{0.25}}$& $81.51_{\pm{3.18}}$& $15.50_{\pm{0.12}}$& $68.29_{\pm{0.29}}$& $80.52_{\pm{0.71}}$& $5.48_{\pm{1.22}}$& $59.50_{\pm{1.82}}$& $14.48_{\pm{0.96}}$ \\
%     \textbf{$1$}& $18.35_{\pm{0.88}}$& $84.28_{\pm{2.20}}$& $15.06_{\pm{0.17}}$& $68.38_{\pm{3.85}}$& $79.62_{\pm{0.23}}$& $6.66_{\pm{2.86}}$& $56.92_{\pm{0.36}}$& $17.96_{\pm{0.70}}$ \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Data selection strategy ablation experiments on the CIFAR-10 dataset with the buffer size of 200, using ER + TRADES as the baseline.
%     When $\rho = 11$, this is equivalent to not applying the robust data selection strategy.}
%     \label{Ablation2}
% \end{table*}

% \begin{table}[]
    
% \centering % 居中显示
%     \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{lllll}
%     \toprule
%     \multirow{2}{*}{\textbf{$\rho$}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{2}{c}{\textbf{Adversarial Data}}\\
%     ~&\textbf{FAA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}\\
%     \midrule
%     \textbf{$11$}& $78.79_{\pm{0.81}}$& $8.10_{\pm{0.97}}$& $51.33_{\pm{2.3}}$& $21.97_{\pm{1.31}}$ \\
%     % \textbf{$11$}& $18.32_{\pm{0.47}}$& $83.37_{\pm{2.82}}$& $15.30_{\pm{0.5}}$& $68.17_{\pm{0.08}}$& $78.97_{\pm{1.06}}$& $7.74_{\pm{1.05}}$& $52.64_{\pm{0.67}}$& $21.81_{\pm{1.82}}$\\
%     \textbf{$10$}& $80.38_{\pm{0.16}}$& $7.06_{\pm{0.93}}$& $59.88_{\pm{1.21}}$& $13.78_{\pm{0.97}}$ \\
%     \textbf{$5$}& $80.52_{\pm{0.71}}$& $5.48_{\pm{1.22}}$& $59.50_{\pm{1.82}}$& $14.48_{\pm{0.96}}$ \\
%     \textbf{$1$}& $79.62_{\pm{0.23}}$& $6.66_{\pm{2.86}}$& $56.92_{\pm{0.36}}$& $17.96_{\pm{0.70}}$ \\
%     \bottomrule
%     \end{tabular}}
%     \caption{Data selection strategy ablation experiments on the CIFAR-10 dataset with the buffer size of 200, using ER + TRADES as the baseline in the task incremental setting.
%     When $\rho = 11$, this is equivalent to not applying the robust data selection strategy.}
%     \label{Ablation2}
% \end{table}

\begin{table}[]
    
\centering % 居中显示
\caption{Data selection strategy ablation experiments on the CIFAR-10 dataset with the buffer size of 200, using ER + TRADES as the baseline in the class/task incremental settings.
    When $\rho = 11$, this is equivalent to not applying the robust data selection strategy.}
    \label{Ablation2_std}
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{lllll}
    \toprule
    \multirow{2}{*}{\textbf{$\rho$}}&
    \multicolumn{2}{c}{\textbf{Class Incremental Setting}}&
    \multicolumn{2}{c}{\textbf{Task Incremental Setting}}\\
    ~&\textbf{FAA$\uparrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{PGD-20$\uparrow$}\\
    \midrule
    \textbf{$11$}&$22.42_{\pm{7.11}}$& $15.72_{\pm{0.82}}$& $78.79_{\pm{0.81}}$& $51.33_{\pm{2.3}}$\\
    % \textbf{$11$}& $18.32_{\pm{0.47}}$& $83.37_{\pm{2.82}}$& $15.30_{\pm{0.5}}$& $68.17_{\pm{0.08}}$& $78.97_{\pm{1.06}}$& $7.74_{\pm{1.05}}$& $52.64_{\pm{0.67}}$& $21.81_{\pm{1.82}}$\\
    \textbf{$10$}& $18.04_{\pm{0.58}}$& $15.31_{\pm{0.18}}$& $80.38_{\pm{0.16}}$& $59.88_{\pm{1.21}}$ \\
    \textbf{$5$}& $18.21_{\pm{0.25}}$& $15.50_{\pm{0.12}}$& $80.52_{\pm{0.71}}$& $59.50_{\pm{1.82}}$\\
    \textbf{$1$}& $18.35_{\pm{0.88}}$ & $15.06_{\pm{0.17}}$& $79.62_{\pm{0.23}}$& $56.92_{\pm{0.36}}$ \\
    \bottomrule
    \end{tabular}}
    
\end{table}

==> Tables/Ablation3_std.tex <==
\begin{table*}[]
    \centering % 居中显示
        \caption{Ablation experiments of different $\alpha$.}
    \label{Ablation3_std}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l ll lll lll}
    \toprule
    \multirow{3}{*}{\textbf{$\alpha$}}&
    \multicolumn{4}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{4}{c}{\textbf{Task Incremental Setting}} \\
    ~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{2}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{2}{c}{\textbf{Adversarial Data}}\\
    ~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&\textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&\textbf{Forgetting$\downarrow$}\\
    \midrule
    
    $0.0$& \pmb{$38.85_{\pm{3.26}}$}& {$47.53_{\pm{21.21}}$}& {$17.56_{\pm{1.40}}$}& {$42.80_{\pm{21.82}}$}& \pmb{$82.70_{\pm{0.43}}$}& \pmb{$9.97_{\pm{1.04}}$} & $50.67_{\pm{6.55}}$& $26.28_{\pm{10.45}}$ \\

    $3.5$& $37.88_{\pm{0.54}}$& $21.76_{\pm{0.23}}$&  \pmb{$18.58_{\pm{1.90}}$}& $21.77_{\pm{0.24}}$& $81.66_{\pm{0.02}}$& $10.86_{\pm{0.78}}$& \pmb{$53.64_{\pm{1.48}}$}& $17.60_{\pm{0.28}}$\\

    $7.0$& $35.92_{\pm{0.88}}$& \pmb{$20.99_{\pm{6.03}}$}& $13.89_{\pm{0.63}}$&  \pmb{$21.76_{\pm{0.67}}$}& $82.56_{\pm{0.58}}$& $10.49_{\pm{3.75}}$& $52.69_{\pm{1.18}}$& \pmb{$16.25_{\pm{2.52}}$}\\

    % $4$& \pmb{$38.85_{\pm{3.26}}$}& \pmb{$47.53_{\pm{21.21}}$}& \pmb{$17.56_{\pm{1.4}}$}& \pmb{$42.80_{\pm{21.82}}$}& \pmb{$82.70_{\pm{0.43}}$}& $9.97_{\pm{1.04}}$& $50.67_{\pm{6.55}}$& $26.28_{\pm{10.45}}$ \\

    % $7$& \pmb{$38.85_{\pm{3.26}}$}& \pmb{$47.53_{\pm{21.21}}$}& \pmb{$17.56_{\pm{1.4}}$}& \pmb{$42.80_{\pm{21.82}}$}& \pmb{$82.70_{\pm{0.43}}$}& $9.97_{\pm{1.04}}$& $50.67_{\pm{6.55}}$& $26.28_{\pm{10.45}}$ \\

    % $10$& \pmb{$38.85_{\pm{3.26}}$}& \pmb{$47.53_{\pm{21.21}}$}& \pmb{$17.56_{\pm{1.4}}$}& \pmb{$42.80_{\pm{21.82}}$}& \pmb{$82.70_{\pm{0.43}}$}& $9.97_{\pm{1.04}}$& $50.67_{\pm{6.55}}$& $26.28_{\pm{10.45}}$ \\
   
\bottomrule
\end{tabular}}

\end{table*}

==> Tables/Acc_per_task.tex <==
\begin{table*}[]
\begin{minipage}{\linewidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lllllll}
    \toprule
    \textbf{Buffer Size}&
    \textbf{Methods}&
    \textbf{Task1}&
    \textbf{Task2}&
    \textbf{Task3}&
    \textbf{Task4}&
    \textbf{Task5}\\
    \midrule
    {\textbf{200}}&\textbf{ER+AT} \\
    ~&\textbf{ER+AT+Ours} \\
    \cmidrule(r){2-7}
    ~&\textbf{ER+TRADES}& $2.83_{\pm{4.15}}$& $1.63_{\pm{1.82}}$& $4.0_{\pm{6.8}}$& $15.68_{\pm{23.91}}$& $87.97_{\pm{1.72}}$ \\
    ~&\textbf{ER+TRADES+Ours}& $48.2_{\pm{12.78}}$& $12.47_{\pm{7.07}}$& $25.72_{\pm{11.47}}$& $51.12_{\pm{16.43}}$& $79.2_{\pm{6.44}}$ \\
    \midrule
    {\textbf{5120}}&\textbf{ER+AT} \\
    ~&\textbf{ER+AT+Ours} \\
    \cmidrule(r){2-7}
    ~&\textbf{ER+TRADES}& $1.77_{\pm{1.53}}$& $0.72_{\pm{1.24}}$& $4.33_{\pm{7.46}}$& $2.42_{\pm{3.97}}$& $92.57_{\pm{0.15}}$ \\
    ~&\textbf{ER+TRADES+Ours}& $26.22_{\pm{26.62}}$& $29.72_{\pm{28.4}}$& $15.12_{\pm{9.97}}$& $37.08_{\pm{11.45}}$& $90.85_{\pm{2.47}}$ \\
    \bottomrule
    \end{tabular}}
    \subcaption{(a)}
    \label{AverageAcc-Clean-CIL-CIFAR10}
\end{minipage}

\begin{minipage}{\linewidth}
    \centering % 居中显示
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lllllll}
    \toprule
    \textbf{Buffer Size}&
    \textbf{Methods}&
    \textbf{Task1}&
    \textbf{Task2}&
    \textbf{Task3}&
    \textbf{Task4}&
    \textbf{Task5}\\
    \midrule
    {\textbf{200}}&\textbf{ER+AT} \\
    ~&\textbf{ER+AT+Ours} \\
    \cmidrule(r){2-7}
    ~&\textbf{ER+TRADES}& $83.77_{\pm{1.73}}$& $63.75_{\pm{1.7}}$& $73.83_{\pm{2.73}}$& $83.92_{\pm{4.86}}$& $88.68_{\pm{1.48}}$ \\
    ~&\textbf{ER+TRADES+Ours}& $88.4_{\pm{1.88}}$& $65.83_{\pm{4.15}}$& $77.6_{\pm{0.69}}$& $89.0_{\pm{2.09}}$& $92.1_{\pm{0.35}}$ \\
    \midrule
    {\textbf{5120}}&\textbf{ER+AT} \\
    ~&\textbf{ER+AT+Ours} \\
    \cmidrule(r){2-7}
    ~&\textbf{ER+TRADES}& $95.75_{\pm{0.48}}$& $78.45_{\pm{2.05}}$& $83.2_{\pm{2.01}}$& $92.33_{\pm{0.99}}$& $92.65_{\pm{0.18}}$ \\
    ~&\textbf{ER+TRADES+Ours}& $87.23_{\pm{9.73}}$& $78.32_{\pm{0.3}}$& $81.85_{\pm{2.09}}$& $91.72_{\pm{0.28}}$& $93.3_{\pm{0.68}}$\\
    \bottomrule
    \end{tabular}}
    \subcaption{(b)}
    \label{AverageAcc-Clean-TIL-CIFAR10}
\end{minipage}
\begin{minipage}{\linewidth}
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lllllll}
    \toprule
    \textbf{Buffer Size}&
    \textbf{Methods}&
    \textbf{Task1}&
    \textbf{Task2}&
    \textbf{Task3}&
    \textbf{Task4}&
    \textbf{Task5}\\
    \midrule
    {\textbf{200}}&\textbf{ER+AT} \\
    ~&\textbf{ER+AT+Ours} \\
    \cmidrule(r){2-7}
    ~&\textbf{ER+TRADES}& $0.48_{\pm{0.71}}$& $0.23_{\pm{0.32}}$& $1.02_{\pm{1.76}}$& $4.57_{\pm{7.87}}$& $72.3_{\pm{7.23}}$ \\
    ~&\textbf{ER+TRADES+Ours}& $22.42_{\pm{7.18}}$& $2.43_{\pm{1.53}}$& $8.3_{\pm{4.38}}$& $19.08_{\pm{10.56}}$& $47.03_{\pm{11.93}}$\\
    \midrule
    {\textbf{5120}}&\textbf{ER+AT} \\
    ~&\textbf{ER+AT+Ours} \\
    \cmidrule(r){2-7}
    ~&\textbf{ER+TRADES}& $0.58_{\pm{0.68}}$& $0.0_{\pm{0.0}}$& $1.05_{\pm{1.82}}$& $0.43_{\pm{0.75}}$& $79.42_{\pm{1.08}}$ \\
    ~&\textbf{ER+TRADES+Ours}& $11.78_{\pm{14.95}}$& $13.67_{\pm{18.89}}$& $4.63_{\pm{3.78}}$& $14.48_{\pm{8.82}}$& $77.07_{\pm{3.79}}$ \\
    \bottomrule
    \end{tabular}}
    \subcaption{(c)}
    \label{AverageAcc-PGD-CIL-CIFAR10}
\end{minipage}

\begin{minipage}{\linewidth}
    \centering % 居中显示
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lllllll}
    \toprule
    \textbf{Buffer Size}&
    \textbf{Methods}&
    \textbf{Task1}&
    \textbf{Task2}&
    \textbf{Task3}&
    \textbf{Task4}&
    \textbf{Task5}\\
    \midrule
    {\textbf{200}}&\textbf{ER+AT} \\
    ~&\textbf{ER+AT+Ours} \\
    \cmidrule(r){2-7}
    ~&\textbf{ER+TRADES}&$57.07_{\pm{3.66}}$& $24.35_{\pm{3.8}}$& $38.43_{\pm{5.16}}$& $60.95_{\pm{2.82}}$& $75.87_{\pm{2.06}}$  \\
    ~&\textbf{ER+TRADES+Ours}& $73.73_{\pm{0.83}}$& $36.1_{\pm{1.53}}$& $47.25_{\pm{3.05}}$& $62.12_{\pm{2.53}}$& $77.83_{\pm{0.41}}$ \\
    \midrule
    {\textbf{5120}}&\textbf{ER+AT} \\
    ~&\textbf{ER+AT+Ours} \\
    \cmidrule(r){2-7}
    ~&\textbf{ER+TRADES}&$78.23_{\pm{1.28}}$& $41.5_{\pm{1.83}}$& $51.43_{\pm{2.4}}$& $70.92_{\pm{0.55}}$& $79.72_{\pm{0.4}}$ \\
    ~&\textbf{ER+TRADES+Ours}& $76.28_{\pm{11.7}}$& $53.83_{\pm{1.73}}$& $60.13_{\pm{2.41}}$& $75.77_{\pm{0.72}}$& $80.27_{\pm{0.31}}$ \\
    \bottomrule
    \end{tabular}}
    \subcaption{(d)}
    \label{AverageAcc-PGD-TIL-CIFAR10}
\end{minipage}

 \caption{Average accuracy of final models on Split-CIFAR10.
 (a) Clean average accuracy of final models on Split-CIFAR10 in the class incremental setting.
 (b) Clean average accuracy of final models on Split-CIFAR10 in the task incremental setting.
 (c) PGD-20 average accuracy of final models on Split-CIFAR10 in the class incremental setting.
 (d) PGD-20 average accuracy of final models on Split-CIFAR10 in the task incremental setting.
 }
\label{AverageAccuracy-CIFAR10}
\end{table*}

==> Tables/Analysis.tex <==
\begin{table*}[t]  
    \centering % 居中显示
     \vspace{-7pt}
\includegraphics[width=\linewidth]{Tables/table.pdf}
\caption{A systematic experimental analysis of the combination of adversarial training (more specifically, Vanilla AT~\cite{madry2018towards}) and memory-based continual learning algorithms. See Sec. 3.2 for a detailed summary of observations. The formula definitions of FAA (final average accuracy), CRD (final average clean relative decrease), FRI (forgetting relative increase), and RRD (final average Robust Relative Decrease compared with the joint model), please see supplementary materials. Adversarial data are generated by PGD-20.
    For convenience, CRD, FRI, and RRD in the table are the averages of task incremental setting and class incremental setting.}
    \label{Analysis} 
\end{table*}

==> Tables/Data_selection_methods_var.tex <==
\begin{table*}[]
    \centering % 居中显示
        \caption{Experiments with other data selection-based and logit masking-based continual learning methods. }
    \label{Data_selection_and_logit_masking_std}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ll ll lll lll}
    \toprule
    \multirow{3}{*}{\textbf{Method}}&\multirow{3}{*}{\textbf{Publication}}
    \multicolumn{4}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{4}{c}{\textbf{Task Incremental Setting}} \\
    ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{2}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{2}{c}{\textbf{Adversarial Data}}\\
    ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&\textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&\textbf{Forgetting$\downarrow$}\\
     \midrule
    ER+AT&\multirow{2}{*}{NeurIPS~$2019$}& $28.18_{\pm{0.69}}$ & $80.58_{\pm{1.05}}$ & $17.86_{\pm{0.29}}$ & $69.58_{\pm{1.15}}$ & $84.49_{\pm{0.61}}$ & $10.23_{\pm{0.98}}$ & $44.30_{\pm{1.05}}$ &$36.89_{\pm{1.11}}$\\

    ER+AT+Ours&~& $47.70_{\pm{0.67}}$&$53.19_{\pm{1.87}}$&$18.20_{\pm{0.02}}$&$56.73_{\pm{1.10}}$&$85.40_{\pm{1.28}}$&$9.20_{\pm{1.67}}$&$48.38_{\pm{0.67}}$&$31.68_{\pm{1.49}}$\\
    \midrule
    
    % GSS+AT&  $27.3_{\pm{0.58}}$& $81.25_{\pm{1.11}}$& $16.85_{\pm{0.18}}$& $68.44_{\pm{0.09}}$& $83.93_{\pm{0.52}}$& $10.54_{\pm{1.11}}$& $43.8_{\pm{0.98}}$& $35.63_{\pm{1.46}}$ \\
    GSS+AT&\multirow{2}{*}{NeurIPS~$2019$}&{$27.59_{\pm{0.62}}$} &{$80.78_{\pm{0.99}}$} &{$16.67_{\pm{0.16}}$} &{$68.53_{\pm{0.11}}$} &{$84.41_{\pm{0.10}}$} &{$9.83_{\pm{0.13}}$} &{$44.25_{\pm{0.87}}$} &$34.79_{\pm{0.09}}$\\
    GSS+AT+Ours&~&{$36.93_{\pm{7.13}}$} &{$67.72_{\pm{15.65}}$} &{$16.84_{\pm{0.01}}$} &{$60.04_{\pm{16.20}}$} &{$85.57_{\pm{0.56}}$} &{$8.86_{\pm{1.84}}$} &{$47.11_{\pm{0.04}}$} &$31.83_{\pm{0.36}}$\\
    \midrule
    ASER+AT&\multirow{2}{*}{AAAI~$2021$}&{$18.85_{\pm{0.00}}$} &{$87.78_{\pm{0.34}}$} &{$14.06_{\pm{0.57}}$} &{$65.57_{\pm{0.01}}$} &{$73.87_{\pm{6.23}}$} &{$19.01_{\pm{13.46}}$} &{$30.65_{\pm{14.44}}$} &$44.85_{\pm{30.80}}$\\
    ASER+AT+Ours&~&{$24.45_{\pm{0.03}}$} &{$81.73_{\pm{0.60}}$} &{$14.91_{\pm{0.07}}$} &{$62.74_{\pm{0.66}}$} &{$77.70_{\pm{0.08}}$} &{$15.21_{\pm{0.43}}$} &{$34.50_{\pm{0.15}}$} &$38.55_{\pm{0.39}}$\\
    \midrule
    X-DER+AT&\multirow{2}{*}{TPAMI~$2022$}&{$34.04_{\pm{0.81}}$} &{$25.13_{\pm{16.25}}$} &{$16.82_{\pm{0.95}}$} &{$27.84_{\pm{17.33}}$} &{$80.80_{\pm{0.44}}$} &{$4.96_{\pm{2.74}}$} &{$60.83_{\pm{0.31}}$} &$10.99_{\pm{0.65}}$\\
    X-DER+AT+Ours&~&{$43.25_{\pm{0.09}}$} &{$20.77_{\pm{2.56}}$} &{$17.22_{\pm{0.00}}$} &{$18.56_{\pm{11.86}}$} &{$84.87_{\pm{0.00}}$} &{$1.74_{\pm{0.02}}$} &{$61.68_{\pm{0.00}}$} &$7.03_{\pm{1.50}}$\\
    
    % ASER+AT&  $14.3_{\pm{1.37}}$& $66.26_{\pm{17.44}}$& $6.14_{\pm{0.78}}$& $40.15_{\pm{62.91}}$& $60.06_{\pm{21.55}}$& $10.3_{\pm{0.65}}$& $17.18_{\pm{11.69}}$& $27.35_{\pm{44.24}}$\\

    % ER-ACE+AT  & $52.11_{\pm{1.31}}$ & $29.35_{\pm{4.13}}$ & $13.99_{\pm{0.30}}$ & $25.92_{\pm{2.97}}$ & $87.37_{\pm{0.24}}$ & $7.76_{\pm{0.08}}$ & $44.65_{\pm{0.81}}$ &$26.74_{\pm{2.34}}$\\

    % XDER+AT  & $45.73_{\pm{4.3}}$& $20.97_{\pm{1.34}}$& $12.28_{\pm{0.81}}$& $18.09_{\pm{2.45}}$& $86.89_{\pm{0.69}}$& $8.08_{\pm{0.53}}$& $46.17_{\pm{3.4}}$& $21.12_{\pm{1.43}}$\\
   
   
\bottomrule
\end{tabular}}
\end{table*}

==> Tables/Main.tex <==
\begin{table*}[]
    \vspace{-8pt}
\begin{minipage}{\linewidth}
    \centering
\includegraphics[0.95\linewidth]{Images/CIFAR10100_new.pdf}
\end{minipage}
    \caption{Experiment results on Split-CIFAR10/100 dataset and model architecture is ResNet18.
    Here PGD-20 and AA are adversarial data Final Average Accuracy (FAA) generated by PGD-20 and Auto Attack (AA) respectively. Forgetting of adversarial data is computed based on PGD-20. \textbf{Bold} represents the best experimental results for the same settings. With the addition of ours, model performance can be improved across the board.}
    \label{MainCIFAR}
\end{table*}



==> Tables/Main_CIFAR100.tex <==
% \begin{table*}[]
%     \caption{Experiment results on Split-CIFAR10 dataset and model architecture is ResNet18.
%     Consistent with the analysis of Table~\ref{Analysis}, we chose two buffer sizes of 200 and 5120.
%     Here PGD-20 and AA are adversarial data Final Average Accuracy (FAA) generated by PGD-20 and Auto Attack (AA) respectively. Forgetting of adversarial data is computed based on PGD-20.}
%     \label{Main-CIFAR10}
%     \centering % 居中显示
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{llllllllllll}
%     \toprule
%     \multirow{3}{*}{\textbf{Buffer Size}} &
%     \multirow{3}{*}{\textbf{Methods}} &
%     \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
%     ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
%     ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{AA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{FAA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{AA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}\\
%     \midrule
%     \multirow{6}{*}{\textbf{200}}&\textbf{ER+AT}& $28.18_{\pm{0.69}}$ & $80.58_{\pm{1.05}}$ & $17.86_{\pm{0.29}}$ &$16.94_{\pm{0.38}}$ & $69.58_{\pm{1.15}}$ & $84.49_{\pm{0.61}}$ & $10.23_{\pm{0.98}}$ & $44.30_{\pm{1.05}}$ & $44.69_{\pm{1.04}}$ & $36.89_{\pm{1.11}}$  \\
%     ~&\textbf{ER+TRADES}& $22.42_{\pm{7.11}}$& $77.25_{\pm{10.79}}$& $15.72_{\pm{0.82}}$& $15.53_{\pm{0.68}}$& $64.95_{\pm{5.58}}$& $78.79_{\pm{0.81}}$& $8.1_{\pm{0.97}}$& $51.33_{\pm{2.3}}$& $51.50_{\pm{2.33}}$& $21.97_{\pm{1
% .31}}$  \\
%     ~&\textbf{ER+FAT}&$33.61_{\pm{6.80}}$ & $69.21_{\pm{8.95}}$ & $15.14_{\pm{0.80}}$ & $14.81_{\pm{0.92}}$ & $49.04_{\pm{7.29}} $& $83.40_{\pm{0.92}}$ & $10.35_{\pm{0.83}}$ & $43.69_{\pm{2.08}}$ & $43.96_{\pm{2.11}}$ & $28.56_{\pm{2.14}}$  \\
%     ~&\textbf{ER+LBGAT}& $25.68_{\pm{0.56}}$& $84.47_{\pm{0.63}}$& $16.65_{\pm{0.11}}$& $16.56_{\pm{0.09}}$& $70.5_{\pm{0.29}}$& $78.19_{\pm{1.17}}$& $18.85_{\pm{1.58}}$& $40.69_{\pm{3.03}}$& $40.73_{\pm{3.15}}$& $40.83_{\pm{3.8}}$\\
%     \cmidrule(r){2-12}
%     ~&\textbf{ER+AT+Ours}& $35.68_{\pm{0.57}}$& $71.18_{\pm{0.66}}$& $18.4_{\pm{0.56}}$& $18.16_{\pm{0.50}}$& $67.85_{\pm{0.72}}$& $84.87_{\pm{0.56}}$& $9.93_{\pm{0.6}}$& $47.3_{\pm{1.31}}$& $47.61_{\pm{1.35}}$& $34.04_{\pm{1.42}}$ \\
%     ~&\textbf{ER+TRADES+Ours}& $43.34_{\pm{4.27}}$ & $33.40_{\pm{11.02}}$ & $19.85_{\pm{1.55}}$ &  $18.35_{\pm{1.14}}$ & $30.78_{\pm{8.84}}$ & $82.59_{\pm{1.12}}$& $7.53_{\pm{1.24}}$ & $59.41_{\pm{0.61}}$ &  $59.59_{\pm{0.64}}$ & $14.16_{\pm{1.29}}$\\
%     \cmidrule(r){1-12}
%     \multirow{6}{*}{\textbf{5120}}&\textbf{ER+AT} & $61.88_{\pm{0.74}}$ & $37.72_{\pm{0.73}}$ & $27.28_{\pm{0.56}}$ & $26.69_{\pm{0.52}}$ & $41.66_{\pm{1.22}}$ & $91.24_{\pm{0.19}}$ & $2.56_{\pm{0.12}}$ & $56.59_{\pm{0.88}}$ & $56.90_{\pm{0.88}}$ & $19.34_{\pm{1.11}}$\\
%     ~&\textbf{ER+TRADES}& $20.36_{\pm{2.81}}$& $85.14_{\pm{4.28}}$& $16.3_{\pm{0.44}}$& $16.18_{\pm{0.35}}$& $72.85_{\pm{1.46}}$& $88.48_{\pm{0.81}}$& $1.59_{\pm{0.86}}$& $64.36_{\pm{0.51}}$& $64.52_{\pm{0.48}}$& $12.47_{\pm{0.37}}$   \\
%     ~&\textbf{ER+FAT}& $54.55_{\pm{6.71}}$& $43.18_{\pm{7.51}}$& $19.68_{\pm{2.54}}$& $18.91_{\pm{2.38}}$& $42.15_{\pm{3.59}}$& $91.5_{\pm{0.53}}$& $2.12_{\pm{0.8}}$& $56.72_{\pm{0.65}}$& $56.87_{\pm{0.70}}$& $14.79_{\pm{1.13}}$  \\
%     ~&\textbf{ER+LBGAT}& $62.45_{\pm{0.46}}$& $37.73_{\pm{0.97}}$& $27.42_{\pm{0.27}}$& $26.66_{\pm{0.33}}$& $47.83_{\pm{0.49}}$& $91.1_{\pm{0.62}}$& $3.25_{\pm{1.06}}$& $56.57_{\pm{1.02}}$& $56.31_{\pm{1.13}}$& $19.38_{\pm{0.84}}$\\
%     \cmidrule(r){2-12}
%     ~&\textbf{ER+AT+Ours}& $64.81_{\pm{0.57}}$& $31.73_{\pm{0.86}}$& $29.46_{\pm{0.25}}$& $28.68_{\pm{0.38}}$& $37.62_{\pm{1.37}}$& $91.6_{\pm{0.21}}$& $2.37_{\pm{0.2}}$& $60.04_{\pm{0.83}}$& $60.34_{\pm{0.87}}$& $16.26_{\pm{0.
% 56}}$ \\
%     ~&\textbf{ER+TRADES+Ours} & $39.8_{\pm{12.23}}$& $44.08_{\pm{18.66}}$& $23.07_{\pm{6.1}}$& $21.98_{\pm{5.41}}$& $41.37_{\pm{11.41}}$& $86.48_{\pm{2.55}}$& $1.71_{\pm{0.62}}$& $69.25_{\pm{2.23}}$ & $69.38_{\pm{2.23}}$&$5.33_{\pm{0.74}}$\\
% \bottomrule
% \end{tabular}}
% \end{table*}




\begin{table*}[]



    \caption{Experiment results on Split-CIFAR100 dataset and model architecture is ResNet18.
    Following~\cite{buzzega2020dark}, we choose two buffer sizes of 500 and 2000.
    Here PGD-20 and AA are adversarial data Final Average Accuracy (FAA) generated by PGD-20 and Auto Attack (AA) respectively. Forgetting of adversarial data is computed based on PGD-20. \textbf{Bold} represents the best experimental results for the same settings. With the addition of ours, model performance can be improved across the board.}
    \label{Main-CIFAR100}
    \centering % 居中显示
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llllllllllll}
    \toprule
    \multirow{3}{*}{\textbf{Buffer Size}} &
    \multirow{3}{*}{\textbf{Methods}} &
    \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
    ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
    ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}\\
    \midrule
    \multirow{6}{*}{\textbf{500}}&\textbf{ER+AT}& $11.94_{\pm{0.74}}$& $73.54_{\pm{0.75}}$& $5.66_{\pm{0.31}}$& $5.54_{\pm{0.31}}$& $38.03_{\pm{0.10}}$& $52.71_{\pm{0.96}}$& $28.44_{\pm{1.11}}$& $17.35_{\pm{0.08}}$& $19.56_{\pm
{0.10}}$& $25.67_{\pm{0.26}}$  \\
    ~&\textbf{ER+TRADES}& $7.59_{\pm{0.08}}$& $68.13_{\pm{0.61}}$& $5.43_{\pm{0.05}}$& $5.11_{\pm{0.06}}$& $44.13_{\pm{0.89}}$& $50.75_{\pm{0.42}}$& $20.22_{\pm{0.49}}$& $26.89_{\pm{0.58}}$& $27.69_{\pm{0.56}}$& $20.34_{\pm{0
.72}}$   \\
    ~&\textbf{ER+FAT}& $11.48_{\pm{0.72}}$& $73.99_{\pm{1.18}}$& $5.35_{\pm{0.26}}$& $5.23_{\pm{0.27}}$& $37.26_{\pm{0.62}}$& $56.1_{\pm{1.23}}$& $24.71_{\pm{1.00}}$& $20.01_{\pm{0.85}}$& $22.99_{\pm{0.91}}$& $22.31_{\pm{1.10}}$  \\
    ~&\textbf{ER+LBGAT}& $11.77_{\pm{0.37}}$& $75.1_{\pm{0.40}}$& $6.16_{\pm{0.11}}$& $5.82_{\pm{0.13}}$& $39.77_{\pm{0.18}}$& $42.02_{\pm{2.36}}$& $26.45_{\pm{0.30}}$& $13.99_{\pm{0.83}}$& $14.43_{\pm{0.97}}$& $23.14_{\pm{0.21}}$ \\
    \cmidrule(r){2-12}
    ~&\textbf{ER+AT+Ours}& \pmb{$17.50_{\pm{0.39}}$}& $66.66_{\pm{0.11}}$& $6.76_{\pm{0.36}}$& \pmb{$6.49_{\pm{0.34}}$}& \pmb{$34.54_{\pm{0.24}}$}& $53.10_{\pm{1.46}}$& $28.59_{\pm{1.51}}$& $17.34_{\pm{0.41}}$& $19.04_{\pm{
0.56}}$& $25.77_{\pm{0.66}}$ \\
    ~&\textbf{ER+TRADES+Ours}& $14.61_{\pm{1.15}}$& \pmb{$62.63_{\pm{2.25}}$}& \pmb{$7.15_{\pm{0.22}}$}& $6.42_{\pm{0.23}}$& $37.49_{\pm{2.31}}$& \pmb{$54.65_{\pm{0.94}}$}&\pmb{ $20.56_{\pm{0.51}}$}&\pmb{$27.72_{\pm{0.94}}$}& \pmb{$28.50_{\pm{0.55}}$}& \pmb{$18.25_{\pm{1.28}}$}  \\
    \cmidrule(r){1-12}
    \multirow{6}{*}{\textbf{2000}}&\textbf{ER+AT}& $18.77_{\pm{0.18}}$& $65.06_{\pm{0.58}}$& $7.20_{\pm{0.18}}$& $7.01_{\pm{0.18}}$& $33.56_{\pm{0.26}}$& $62.01_{\pm{0.76}}$& $17.97_{\pm{0.80}}$& $21.16_{\pm{0.38}}$& $24.04_{\pm{
0.23}}$& $20.47_{\pm{0.25}}$ \\
    ~&\textbf{ER+TRADES}& $9.50_{\pm{0.24}}$& $70.49_{\pm{0.38}}$& $5.35_{\pm{0.19}}$& $5.01_{\pm{0.17}}$& $42.08_{\pm{0.40}}$& $60.63_{\pm{1.03}}$& $13.78_{\pm{0.90}}$& $26.68_{\pm{0.51}}$& $29.19_{\pm{0.70}}$& $18.60_{\pm{0.54}
}$   \\
    ~&\textbf{ER+FAT}& $17.09_{\pm{1.96}}$& $66.91_{\pm{3.02}}$& $6.12_{\pm{0.40}}$& $5.93_{\pm{0.38}}$& $33.62_{\pm{1.72}}$& $63.88_{\pm{0.02}}$& $15.99_{\pm{0.47}}$& $23.48_{\pm{0.06}}$& $26.75_{\pm{0.05}}$& $17.12_{\pm{0.62}}$  \\
    ~&\textbf{ER+LBGAT}& $20.58_{\pm{0.15}}$& $63.31_{\pm{0.20}}$& $7.93_{\pm{0.17}}$& $7.05_{\pm{0.16}}$& $30.09_{\pm{0.32}}$& $55.77_{\pm{0.23}}$& $25.11_{\pm{0.54}}$& $17.95_{\pm{0.43}}$& $18.88_{\pm{0.54
}}$& $19.18_{\pm{0.48}}$\\
    \cmidrule(r){2-12}
    ~&\textbf{ER+AT+Ours}& \pmb{$24.52_{\pm{0.37}}$}& \pmb{$57.28_{\pm{0.34}}$}& \pmb{$8.58_{\pm{0.24}}$}& \pmb{$8.25_{\pm{0.25}}$}& \pmb{$28.44_{\pm{0.18}}$}& $62.42_{\pm{0.28}}$& $18.06_{\pm{0.21}}$& $21.28_{\pm{0.05}}$& $23.88_{\p
m{0.21}}$& $20.43_{\pm{0.48}}$\\
    ~&\textbf{ER+TRADES+Ours}& $19.26_{\pm{0.38}}$& $58.26_{\pm{0.87}}$& $8.26_{\pm{0.14}}$& $7.56_{\pm{0.15}}$& $36.67_{\pm{0.14}}$& \pmb{$63.45_{\pm{0.21}}$}& \pmb{$11.32_{\pm{0.41}}$}& \pmb{$31.66_{\pm{0.21}}$}& \pmb{$33.51_{\pm{0.30}}$}& \pmb{$14.26_{\pm{0.41}}$}  \\
    \bottomrule
    \end{tabular}}

\end{table*}






% \begin{table*}[]
%     \caption{The}
%     \label{Main-CIFAR100}
%     \centering % 居中显示
%     \scalebox{0.6}{
%     \begin{tabular}{lllllllllllll}
%     \toprule
%     \multirow{3}{*}{\textbf{Dataset}} &
%     \multirow{3}{*}{\textbf{Buffer Size}} &
%     \multirow{3}{*}{\textbf{Methods}} &
%     \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
%     ~&~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
%     ~&~&~&\textbf{FAA }&\textbf{Forgetting}&
%     \textbf{PGD-20}&
%     \textbf{AA}&
%     \textbf{Forgetting}&
%     \textbf{FAA }&\textbf{Forgetting}&
%     \textbf{PGD-20 }&
%     \textbf{AA}&
%     \textbf{Forgetting}\\
%     \midrule
%     \multirow{12}{*}{\textbf{Split-CIFAR10}}&\multirow{6}{*}{\textbf{200}}&\textbf{ER+AT}& $28.18_{\pm{0.69}}$ & $80.58_{\pm{1.05}}$ & $17.86_{\pm{0.29}}$ &$16.94_{\pm{0.38}}$ & $69.58_{\pm{1.15}}$ & $84.49_{\pm{0.61}}$ & $10.23_{\pm{0.98}}$ & $44.30_{\pm{1.05}}$ & $44.69_{\pm{1.04}}$ & $36.89_{\pm{1.11}}$  \\
%     ~&~&\textbf{ER+TRADES}& $22.42_{\pm{7.11}}$& $77.25_{\pm{10.79}}$& $15.72_{\pm{0.82}}$& $0_{\pm{0}}$& $64.95_{\pm{5.58}}$& $78.79_{\pm{0.81}}$& $8.1_{\pm{0.97}}$& $51.33_{\pm{2.3}}$& $0_{\pm{0}}$& $21.97_{\pm{1
% .31}}$  \\
%     ~&~&\textbf{ER+FAT}&$33.61_{\pm{6.80}}$ & $69.21_{\pm{8.95}}$ & $15.14_{\pm{0.80}}$ & 0 & $49.04_{\pm{7.29}) $& $83.40_{\pm{0.92}}$ & $10.35_{\pm{0.83}}$ & $43.69_{\pm{2.08}}$ & 0 & $28.56_{\pm{2.14}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \cmidrule(r){2-13}
%     ~&\multirow{6}{*}{\textbf{5120}}&\textbf{ER+AT} & $61.88_{\pm{0.74}}$ & $37.72_{\pm{0.73}}$ & $31.27_{\pm{0.63}}$ & $26.69_{\pm{0.52}}$ & $41.66_{\pm{1.22}}$ & $91.24_{\pm{0.19}}$ & $2.56_{\pm{0.12}}$ & $56.59_{\pm{0.88}}$ & $56.90_{\pm{0.88}}$ & $19.34_{\pm{1.11}}$\\
%     ~&~&\textbf{ER+TRADES}& $20.36_{\pm{2.81}}$& $85.14_{\pm{4.28}}$& $16.3_{\pm{0.44}}$& $0_{\pm{0}}$& $72.85_{\pm{1.46}}$& $88.48_{\pm{0.81}}$& $1.59_{\pm{0.86}}$& $64.36_{\pm{0.51}}$& $0_{\pm{0}}$& $12.47_{\pm{0
% .37}}$   \\
%     ~&~&\textbf{ER+FAT}& $54.55_{\pm{6.71}}$& $43.18_{\pm{7.51}}$& $19.68_{\pm{2.54}}$& $0_{\pm{0}}$& $42.15_{\pm{3.59}}$& $91.5_{\pm{0.53}}$& $2.12_{\pm{0.8}}$& $56.72_{\pm{0.65}}$& $0_{\pm{0}}$& $14.79_{\pm{1.
% 13}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \midrule
%     \multirow{12}{*}{\textbf{Split-CIFAR100}}&\multirow{6}{*}{\textbf{500}}&\textbf{ER+AT}&$11.72_{\pm{0.44}}$ & $74.22_{\pm{0.36}}$ & $6.01_{\pm{0.23}}$ & 0 & $37.47_{\pm{0.44}}$ & $54.53_{\pm{1.03}}$& $26.84_{\pm{0.88}}$ & $18.36_{\pm{0.43}}$ & 0 & $24.42_{\pm{0.74}}$  \\
%     ~&~&\textbf{ER+TRADES}& $7.59_{\pm{0.08}}$& $68.13_{\pm{0.61}}$& $5.43_{\pm{0.05}}$& $0_{\pm{0}}$& $44.13_{\pm{0.89}}$& $50.75_{\pm{0.42}}$& $20.22_{\pm{0.49}}$& $26.89_{\pm{0.58}}$& $0_{\pm{0}}$& $20.34_{\pm{0
% .72}}$   \\
%     ~&~&\textbf{ER+FAT}& $11.48_{\pm{0.72}}$& $73.99_{\pm{1.18}}$& $5.35_{\pm{0.26}}$& $0_{\pm{0}}$& $37.26_{\pm{0.62}}$& $56.1_{\pm{1.23}}$& $24.71_{\pm{1.0}}$& $20.01_{\pm{0.85}}$& $0_{\pm{0}}$& $22.31_{\pm{1.
% 1}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \cmidrule(r){2-13}
%     ~&\multirow{6}{*}{\textbf{2000}}&\textbf{ER+AT}& $15.45_{\pm{1.18}}$& $70.15_{\pm{1.24}}$& $6.08_{\pm{0.04}}$& $0_{\pm{0}}$& $36.35_{\pm{0.27}}$& $64.25_{\pm{0.15}}$& $16.34_{\pm{0.16}}$& $22.77_{\pm{0.68}}$& $0_{\pm{0}}$& $19.0_{\pm{0
% .59}}$  \\
%     ~&~&\textbf{ER+TRADES}& $9.5_{\pm{0.24}}$& $70.49_{\pm{0.38}}$& $5.35_{\pm{0.19}}$& $0_{\pm{0}}$& $42.08_{\pm{0.4}}$& $60.63_{\pm{1.03}}$& $13.78_{\pm{0.9}}$& $26.68_{\pm{0.51}}$& $0_{\pm{0}}$& $18.6_{\pm{0.54}
% }$   \\
%     ~&~&\textbf{ER+FAT}& $17.09_{\pm{1.96}}$& $66.91_{\pm{3.02}}$& $6.12_{\pm{0.4}}$& $0_{\pm{0}}$& $33.62_{\pm{1.72}}$& $63.88_{\pm{0.02}}$& $15.99_{\pm{0.47}}$& $23.48_{\pm{0.06}}$& $0_{\pm{0}}$& $17.12_{\pm{0
% .62}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
% \bottomrule
% \end{tabular}}
% \end{table*}

==> Tables/Main_CIFAR_var.tex <==
\begin{table*}[]
    \caption{Experiment results on Split-CIFAR10/100 dataset and model architecture is ResNet18.
    Here PGD-20 and AA are adversarial data Final Average Accuracy (FAA) generated by PGD-20 and Auto Attack (AA) respectively. Forgetting of adversarial data is computed based on PGD-20. With the addition of ours, model performance can be improved across the board.}
    \label{MainCIFAR-var}
\begin{minipage}{\linewidth}
    \centering
    \subcaption{Results on Split-CIFAR10. We chose two buffer sizes of $200$ and $5120$.}
    \label{Main-CIFAR10-var}
    \centering % 居中显示
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llllllllllll}
    \toprule
    \multirow{3}{*}{\textbf{Buffer Size}} &
    \multirow{3}{*}{\textbf{Methods}} &
    \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
    ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
    ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}\\
    \midrule
    \multirow{6}{*}{\textbf{200}}&\textbf{ER+AT}& $28.18_{\pm{0.69}}$ & $80.58_{\pm{1.05}}$ & $17.86_{\pm{0.29}}$ &$16.94_{\pm{0.38}}$ & $69.58_{\pm{1.15}}$ & $84.49_{\pm{0.61}}$ & $10.23_{\pm{0.98}}$ & $44.30_{\pm{1.05}}$ & $44.69_{\pm{1.04}}$ & $36.89_{\pm{1.11}}$  \\
    ~&\textbf{ER+TRADES}& $22.42_{\pm{7.11}}$& $77.25_{\pm{10.79}}$& $15.72_{\pm{0.82}}$& $15.53_{\pm{0.68}}$& $64.95_{\pm{5.58}}$& $78.79_{\pm{0.81}}$& $8.10_{\pm{0.97}}$& $51.33_{\pm{2.30}}$& $51.50_{\pm{2.33}}$& $21.97_{\pm{1
.31}}$  \\
    ~&\textbf{ER+FAT}&$33.61_{\pm{6.80}}$ & $69.21_{\pm{8.95}}$ & $15.14_{\pm{0.80}}$ & $14.81_{\pm{0.92}}$ & $49.04_{\pm{7.29}} $& $83.40_{\pm{0.92}}$ & $10.35_{\pm{0.83}}$ & $43.69_{\pm{2.08}}$ & $43.96_{\pm{2.11}}$ & $28.56_{\pm{2.14}}$  \\
 ~&\textbf{ER+LBGAT}& $25.68_{\pm{0.56}}$& $84.47_{\pm{0.63}}$& $16.65_{\pm{0.11}}$& $16.56_{\pm{0.09}}$& $70.5_{\pm{0.29}}$& $78.19_{\pm{1.17}}$& $18.85_{\pm{1.58}}$& $40.69_{\pm{3.03}}$& $40.73_{\pm{3.15}}$& $40.83_{\pm{3.80}}$\\
 ~&\textbf{ER+Pang~\etal~\cite{pang2022robustness}}&  {$48.65_{\pm{1.76}}$} & $56.79_{\pm{1.78}}$& $2.40_{\pm{0.46}}$& $0.93_{\pm{0.03}}$& $18.96_{\pm{2.47}}$& $88.90_{\pm{2.02}}$& $9.82_{\pm{2.53}}$& $7.25_{\pm{1.06}}$& $6.72_{\pm{0.55}}$& $8.70_{\pm{0.06}}$ \\
    \cmidrule(r){2-12}
    ~&\textbf{ER+AT+Ours}& 
    $35.68_{\pm{0.57}}$& $71.18_{\pm{0.66}}$& $18.40_{\pm{0.56}}$& $18.16_{\pm{0.50}}$& $67.85_{\pm{0.72}}$&  {$84.87_{\pm{0.56}}$}& $9.93_{\pm{0.60}}$& $47.30_{\pm{1.31}}$& $47.61_{\pm{1.35}}$& $34.04_{\pm{1.42}}$ \\
    % $47.70_{\pm{0.67}}$&$53.19_{\pm{1.87}}$&$18.20_{\pm{0.02}}$&$17.48_{\pm{0.01}}$&$56.73_{\pm{1.10}}$&$85.40_{\pm{1.28}}$&$9.20_{\pm{1.67}}$&$48.38_{\pm{0.67}}$&$48.54_{\pm{0.75}}$&$31.68_{\pm{1.49}}$\\
    ~&\textbf{ER+TRADES+Ours}& 
    % $42.72_{\pm{0.14}}$&$26.26_{\pm{2.78}}$&$19.73_{\pm{0.64}}$&$17.54_{\pm{0.02}}$&$23.14_{\pm{5.2}}$&$80.64_{\pm{2.45}}$&$9.25_{\pm{1.38}}$&$58.21_{\pm{0.05}}$&$58.53_{\pm{0.01}}$&$15.57_{\pm{0.0}}$\\
     {$43.34_{\pm{4.27}}$} &  {$33.40_{\pm{11.02}}$} &  {$19.85_{\pm{1.55}}$}&   {$18.35_{\pm{1.14}}$} &  {$30.78_{\pm{8.84}}$}& $82.59_{\pm{1.12}}$& { $7.53_{\pm{1.24}}$ }& { $59.41_{\pm{0.61}}$} &   {$59.59_{\pm{0.64}}$ }&  {$14.16_{\pm{1.29}}$}\\
    \cmidrule(r){1-12}
    \multirow{6}{*}{\textbf{5120}}&\textbf{ER+AT} & $61.88_{\pm{0.74}}$ & $37.72_{\pm{0.73}}$ & $27.28_{\pm{0.56}}$ & $26.69_{\pm{0.52}}$ & $41.66_{\pm{1.22}}$ & $91.24_{\pm{0.19}}$ & $2.56_{\pm{0.12}}$ & $56.59_{\pm{0.88}}$ & $56.90_{\pm{0.88}}$ & $19.34_{\pm{1.11}}$\\
    ~&\textbf{ER+TRADES}& $20.36_{\pm{2.81}}$& $85.14_{\pm{4.28}}$& $16.3_{\pm{0.44}}$& $16.18_{\pm{0.35}}$& $72.85_{\pm{1.46}}$& $88.48_{\pm{0.81}}$&  {$1.59_{\pm{0.86}}$} & $64.36_{\pm{0.51}}$& $64.52_{\pm{0.48}}$& $12.47_{\pm{0.37}}$   \\
    ~&\textbf{ER+FAT}& $54.55_{\pm{6.71}}$& $43.18_{\pm{7.51}}$& $19.68_{\pm{2.54}}$& $18.91_{\pm{2.38}}$& $42.15_{\pm{3.59}}$& $91.50_{\pm{0.53}}$& $2.12_{\pm{0.80}}$& $56.72_{\pm{0.65}}$& $56.87_{\pm{0.70}}$& $14.79_{\pm{1.13}}$  \\
    ~&\textbf{ER+LBGAT}& $62.45_{\pm{0.46}}$& $37.73_{\pm{0.97}}$& $27.42_{\pm{0.27}}$& $26.66_{\pm{0.33}}$& $47.83_{\pm{0.49}}$& $91.10_{\pm{0.62}}$& $3.25_{\pm{1.06}}$& $56.57_{\pm{1.02}}$& $56.31_{\pm{1.13}}$& $19.38_{\pm{0.84}}$\\
   ~&\textbf{ER+Pang~\etal~\cite{pang2022robustness}}& $51.37_{\pm{6.44}}$& $52.84_{\pm{8.47}}$& $3.14_{\pm{0.49}}$&$1.10_{\pm{0.05}}$& $20.29_{\pm{2.92}}$& $95.63_{\pm{0.17}}$& $1.58_{\pm{0.21}}$& $14.66_{\pm{0.15}}$&$13.92_{\pm{0.04}}$& $2.53_{\pm{0.46}}$\\
    \cmidrule(r){2-12}
    ~&\textbf{ER+AT+Ours}& 
    $64.34_{\pm{0.68}}$&$23.64_{\pm{0.23}}$&$31.31_{\pm{0.07}}$&$30.49_{\pm{0.06}}$&$20.46_{\pm{0.75}}$&$91.0_{\pm{0.07}}$&$3.51_{\pm{0.14}}$&$60.49_{\pm{0.24}}$&$60.61_{\pm{0.28}}$&$13.27_{\pm{0.33}}$\\
%      {$64.81_{\pm{0.57}}$}&  {$31.73_{\pm{0.86}}$}&  {$29.46_{\pm{0.25}}$}&  {$28.68_{\pm{0.38}}$}&  {$37.62_{\pm{1.37}}$}&  {$91.60_{\pm{0.21}}$}& $2.37_{\pm{0.20}}$& $60.04_{\pm{0.83}}$& $60.34_{\pm{0.87}}$& $16.26_{\pm{0.
% 56}}$ \\
   ~&\textbf{ER+TRADES+Ours} & 
% $42.12_{\pm{0.88}}$&$1.57_{\pm{1.67}}$&$28.37_{\pm{0.09}}$&$30.33_{\pm{1.78}}$&$1.48_{\pm{0.43}}$&$85.55_{\pm{0.01}}$&$7.02_{\pm{0.04}}$&$67.88_{\pm{0.03}}$&$67.97_{\pm{0.04}}$&$3.81_{\pm{2.33}}$\\
   $39.80_{\pm{12.23}}$& $44.08_{\pm{18.66}}$& $23.07_{\pm{6.10}}$& $21.98_{\pm{5.41}}$& $41.37_{\pm{11.41}}$& $86.48_{\pm{2.55}}$& $1.71_{\pm{0.62}}$&  {$69.25_{\pm{2.23}}$} &  {$69.38_{\pm{2.23}}$} & {$5.33_{\pm{0.74}}$}\\
\bottomrule
\end{tabular}}
\end{minipage}
 
\begin{minipage}{\linewidth}
    \subcaption{Results on Split-CIFAR100. We choose two buffer sizes of $500$ and $2000$.}
    \label{Main-CIFAR100-var}
    \centering % 居中显示
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llllllllllll}
    \toprule
    \multirow{3}{*}{\textbf{Buffer Size}} &
    \multirow{3}{*}{\textbf{Methods}} &
    \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
    ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
    ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}\\
    \midrule
    \multirow{6}{*}{\textbf{500}}&\textbf{ER+AT}& $11.94_{\pm{0.74}}$& $73.54_{\pm{0.75}}$& $5.66_{\pm{0.31}}$& $5.54_{\pm{0.31}}$& $38.03_{\pm{0.10}}$& $52.71_{\pm{0.96}}$& $28.44_{\pm{1.11}}$& $17.35_{\pm{0.08}}$& $19.56_{\pm
{0.10}}$& $25.67_{\pm{0.26}}$  \\
    ~&\textbf{ER+TRADES}& $7.59_{\pm{0.08}}$& $68.13_{\pm{0.61}}$& $5.43_{\pm{0.05}}$& $5.11_{\pm{0.06}}$& $44.13_{\pm{0.89}}$& $50.75_{\pm{0.42}}$& $20.22_{\pm{0.49}}$& $26.89_{\pm{0.58}}$& $27.69_{\pm{0.56}}$& $20.34_{\pm{0
.72}}$   \\
    ~&\textbf{ER+FAT}& $11.48_{\pm{0.72}}$& $73.99_{\pm{1.18}}$& $5.35_{\pm{0.26}}$& $5.23_{\pm{0.27}}$& $37.26_{\pm{0.62}}$& $56.1_{\pm{1.23}}$& $24.71_{\pm{1.00}}$& $20.01_{\pm{0.85}}$& $22.99_{\pm{0.91}}$& $22.31_{\pm{1.10}}$  \\
    ~&\textbf{ER+LBGAT}& $11.77_{\pm{0.37}}$& $75.1_{\pm{0.40}}$& $6.16_{\pm{0.11}}$& $5.82_{\pm{0.13}}$& $39.77_{\pm{0.18}}$& $42.02_{\pm{2.36}}$& $26.45_{\pm{0.30}}$& $13.99_{\pm{0.83}}$& $14.43_{\pm{0.97}}$& $23.14_{\pm{0.21}}$ \\
    ~&\textbf{ER+Pang~\etal~\cite{pang2022robustness}}& $16.22_{\pm{0.63}}$& $77.71_{\pm{0.44}}$& $0.91_{\pm{0.05}}$& $0.62_{\pm{0.00}}$& $6.13_{\pm{0.16}}$& $68.87_{\pm{0.25}}$& $11.21_{\pm{0.73}}$& $3.23_{\pm{0.42}}$& $7.95_{\pm{0.06}}$& $4.94_{\pm{0.05}}$\\

    \cmidrule(r){2-12}
    ~&\textbf{ER+AT+Ours}& 
    $24.14_{\pm{0.44}}$&$53.03_{\pm{0.3}}$&$7.13_{\pm{0.05}}$&$6.68_{\pm{0.04}}$&$25.81_{\pm{0.13}}$&$56.0_{\pm{0.05}}$&$26.19_{\pm{0.03}}$&$17.95_{\pm{0.04}}$&$20.26_{\pm{0.06}}$&$24.87_{\pm{0.08}}$\\
%      {$17.50_{\pm{0.39}}$}& $66.66_{\pm{0.11}}$& $6.76_{\pm{0.36}}$&  {$6.49_{\pm{0.34}}$}&  {$34.54_{\pm{0.24}}$}& $53.10_{\pm{1.46}}$& $28.59_{\pm{1.51}}$& $17.34_{\pm{0.41}}$& $19.04_{\pm{
% 0.56}}$& $25.77_{\pm{0.66}}$ \\
    ~&\textbf{ER+TRADES+Ours}& 
     {$23.24_{\pm{0.01}}$} & {$24.29_{\pm{0.0}}$} & {$9.93_{\pm{0.37}}$} & {$7.5_{\pm{0.37}}$} & {$11.7_{\pm{3.32}}$} & {$56.68_{\pm{0.44}}$} & {$21.39_{\pm{0.12}}$} & {$27.39_{\pm{0.41}}$} & {$28.5_{\pm{0.34}}$} & {$16.76_{\pm{0.22}}$} \\

    % $14.61_{\pm{1.15}}$&  {$62.63_{\pm{2.25}}$}&  {$7.15_{\pm{0.22}}$}& $6.42_{\pm{0.23}}$& $37.49_{\pm{2.31}}$&  {$54.65_{\pm{0.94}}$}& { $20.56_{\pm{0.51}}$}& {$27.72_{\pm{0.94}}$}&  {$28.50_{\pm{0.55}}$}&  {$18.25_{\pm{1.28}}$}  \\
    \cmidrule(r){1-12}
    \multirow{6}{*}{\textbf{2000}}&\textbf{ER+AT}& $18.77_{\pm{0.18}}$& $65.06_{\pm{0.58}}$& $7.20_{\pm{0.18}}$& $7.01_{\pm{0.18}}$& $33.56_{\pm{0.26}}$& $62.01_{\pm{0.76}}$& $17.97_{\pm{0.80}}$& $21.16_{\pm{0.38}}$& $24.04_{\pm{
0.23}}$& $20.47_{\pm{0.25}}$ \\
    ~&\textbf{ER+TRADES}& $9.50_{\pm{0.24}}$& $70.49_{\pm{0.38}}$& $5.35_{\pm{0.19}}$& $5.01_{\pm{0.17}}$& $42.08_{\pm{0.40}}$& $60.63_{\pm{1.03}}$& $13.78_{\pm{0.90}}$& $26.68_{\pm{0.51}}$& $29.19_{\pm{0.70}}$& $18.60_{\pm{0.54}
}$   \\
    ~&\textbf{ER+FAT}& $17.09_{\pm{1.96}}$& $66.91_{\pm{3.02}}$& $6.12_{\pm{0.40}}$& $5.93_{\pm{0.38}}$& $33.62_{\pm{1.72}}$& $63.88_{\pm{0.02}}$& $15.99_{\pm{0.47}}$& $23.48_{\pm{0.06}}$& $26.75_{\pm{0.05}}$& $17.12_{\pm{0.62}}$  \\
    ~&\textbf{ER+LBGAT}& $20.58_{\pm{0.15}}$& $63.31_{\pm{0.20}}$& $7.93_{\pm{0.17}}$& $7.05_{\pm{0.16}}$& $30.09_{\pm{0.32}}$& $55.77_{\pm{0.23}}$& $25.11_{\pm{0.54}}$& $17.95_{\pm{0.43}}$& $18.88_{\pm{0.54
}}$& $19.18_{\pm{0.48}}$\\
~&\textbf{ER+Pang~\etal~\cite{pang2022robustness}}& $30.10_{\pm{0.53}}$& $61.51_{\pm{1.00}}$& $0.75_{\pm{0.22}}$&$0.51_{\pm{0.02}}$& $4.10_{\pm{0.60}}$& $76.90_{\pm{0.44}}$& $19.60_{\pm{0.32}}$& $4.88_{\pm{0.24}}$&$11.97_{\pm{0.26}}$& $5.25_{\pm{0.20}}$\\
    \cmidrule(r){2-12}
    ~&\textbf{ER+AT+Ours}& 
    $31.93_{\pm{0.07}}$&$40.5_{\pm{0.12}}$&$9.61_{\pm{0.06}}$&$9.16_{\pm{0.04}}$&$17.78_{\pm{0.22}}$&$63.77_{\pm{0.18}}$&$17.16_{\pm{0.31}}$&$23.11_{\pm{0.02}}$&$25.59_{\pm{0.08}}$&$17.57_{\pm{0.07}}$\\
%      {$24.52_{\pm{0.37}}$}&  {$57.28_{\pm{0.34}}$}&  {$8.58_{\pm{0.24}}$}&  {$8.25_{\pm{0.25}}$}&  {$28.44_{\pm{0.18}}$}& $62.42_{\pm{0.28}}$& $18.06_{\pm{0.21}}$& $21.28_{\pm{0.05}}$& $23.88_{\p
% m{0.21}}$& $20.43_{\pm{0.48}}$\\
    ~&\textbf{ER+TRADES+Ours}&
    $28.73_{\pm{1.79}}$&$24.16_{\pm{2.6}}$&$12.75_{\pm{0.34}}$&$11.02_{\pm{0.66}}$&$14.56_{\pm{0.7}}$&$62.01_{\pm{0.89}}$&$13.16_{\pm{1.9}}$&$34.81_{\pm{0.41}}$&$35.36_{\pm{0.95}}$&$11.6_{\pm{0.17}}$\\
    % $19.26_{\pm{0.38}}$& $58.26_{\pm{0.87}}$& $8.26_{\pm{0.14}}$& $7.56_{\pm{0.15}}$& $36.67_{\pm{0.14}}$&  {$63.45_{\pm{0.21}}$}&  {$11.32_{\pm{0.41}}$}&  {$31.66_{\pm{0.21}}$}&  {$33.51_{\pm{0.30}}$}&  {$14.26_{\pm{0.41}}$}  \\
    \bottomrule
    \end{tabular}}
\end{minipage}



\end{table*}




% \begin{table*}[]
%     \caption{Experiment results on Split-CIFAR100 dataset and model architecture is ResNet18.
%     Following~\cite{buzzega2020dark}, we choose two buffer sizes of 500 and 2000.
%     Here PGD-20 and AA are adversarial data Final Average Accuracy (FAA) generated by PGD-20 and Auto Attack (AA) respectively. Forgetting of adversarial data is computed based on PGD-20.}
%     \label{Main-CIFAR100}
%     \centering % 居中显示
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{llllllllllll}
%     \toprule
%     \multirow{3}{*}{\textbf{Buffer Size}} &
%     \multirow{3}{*}{\textbf{Methods}} &
%     \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
%     ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
%     ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{AA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{FAA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{AA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}\\
%     \midrule
%     \multirow{6}{*}{\textbf{500}}&\textbf{ER+AT}& $11.94_{\pm{0.74}}$& $73.54_{\pm{0.75}}$& $5.66_{\pm{0.31}}$& $5.54_{\pm{0.31}}$& $38.03_{\pm{0.1}}$& $52.71_{\pm{0.96}}$& $28.44_{\pm{1.11}}$& $17.35_{\pm{0.08}}$& $19.56_{\pm
% {0.1}}$& $25.67_{\pm{0.26}}$  \\
%     ~&\textbf{ER+TRADES}& $7.59_{\pm{0.08}}$& $68.13_{\pm{0.61}}$& $5.43_{\pm{0.05}}$& $5.11_{\pm{0.06}}$& $44.13_{\pm{0.89}}$& $50.75_{\pm{0.42}}$& $20.22_{\pm{0.49}}$& $26.89_{\pm{0.58}}$& $27.69_{\pm{0.56}}$& $20.34_{\pm{0
% .72}}$   \\
%     ~&\textbf{ER+FAT}& $11.48_{\pm{0.72}}$& $73.99_{\pm{1.18}}$& $5.35_{\pm{0.26}}$& $5.23_{\pm{0.27}}$& $37.26_{\pm{0.62}}$& $56.1_{\pm{1.23}}$& $24.71_{\pm{1.00}}$& $20.01_{\pm{0.85}}$& $22.99_{\pm{0.91}}$& $22.31_{\pm{1.10}}$  \\
%     ~&\textbf{ER+LBGAT}& $11.77_{\pm{0.37}}$& $75.1_{\pm{0.4}}$& $6.16_{\pm{0.11}}$& $5.82_{\pm{0.13}}$& $39.77_{\pm{0.18}}$& $42.02_{\pm{2.36}}$& $26.45_{\pm{0.3}}$& $13.99_{\pm{0.83}}$& $14.43_{\pm{0.97}}$& $23.14_{\pm{0.21}}$ \\
%     \cmidrule(r){2-12}
%     ~&\textbf{ER+AT+Ours}& $17.5_{\pm{0.39}}$& $66.66_{\pm{0.11}}$& $6.76_{\pm{0.36}}$& $6.49_{\pm{0.34}}$& $34.54_{\pm{0.24}}$& $53.1_{\pm{1.46}}$& $28.59_{\pm{1.51}}$& $17.34_{\pm{0.41}}$& $19.04_{\pm{
% 0.56}}$& $25.77_{\pm{0.66}}$ \\
%     ~&\textbf{ER+TRADES+Ours}& $14.61_{\pm{1.15}}$& $62.63_{\pm{2.25}}$& $7.15_{\pm{0.22}}$& $6.42_{\pm{0.23}}$& $37.49_{\pm{2.31}}$& $54.65_{\pm{0.94}}$& $20.56_{\pm{0.51}}$& $27.72_{\pm{0.94}}$& $28.50_{\pm{0.55}}$& $18.25_{\pm{1.28}}$  \\
%     \cmidrule(r){1-12}
%     \multirow{6}{*}{\textbf{2000}}&\textbf{ER+AT}& $18.77_{\pm{0.18}}$& $65.06_{\pm{0.58}}$& $7.2_{\pm{0.18}}$& $7.01_{\pm{0.18}}$& $33.56_{\pm{0.26}}$& $62.01_{\pm{0.76}}$& $17.97_{\pm{0.8}}$& $21.16_{\pm{0.38}}$& $24.04_{\pm{
% 0.23}}$& $20.47_{\pm{0.25}}$ \\
%     ~&\textbf{ER+TRADES}& $9.50_{\pm{0.24}}$& $70.49_{\pm{0.38}}$& $5.35_{\pm{0.19}}$& $5.01_{\pm{0.17}}$& $42.08_{\pm{0.4}}$& $60.63_{\pm{1.03}}$& $13.78_{\pm{0.9}}$& $26.68_{\pm{0.51}}$& $29.19_{\pm{0.70}}$& $18.6_{\pm{0.54}
% }$   \\
%     ~&\textbf{ER+FAT}& $17.09_{\pm{1.96}}$& $66.91_{\pm{3.02}}$& $6.12_{\pm{0.4}}$& $5.93_{\pm{0.38}}$& $33.62_{\pm{1.72}}$& $63.88_{\pm{0.02}}$& $15.99_{\pm{0.47}}$& $23.48_{\pm{0.06}}$& $26.75_{\pm{0.05}}$& $17.12_{\pm{0.62}}$  \\
%     ~&\textbf{ER+LBGAT}& $20.58_{\pm{0.15}}$& $63.31_{\pm{0.2}}$& $7.93_{\pm{0.17}}$& $0.0_{\pm{0.0}}$& $30.09_{\pm{0.32}}$& $55.77_{\pm{0.23}}$& $25.11_{\pm{0.54}}$& $17.95_{\pm{0.43}}$& $0.0_{\pm{0.0
% }}$& $19.18_{\pm{0.48}}$\\
%     \cmidrule(r){2-12}
%     ~&\textbf{ER+AT+Ours}& $24.52_{\pm{0.37}}$& $57.28_{\pm{0.34}}$& $8.58_{\pm{0.24}}$& $8.25_{\pm{0.25}}$& $28.44_{\pm{0.18}}$& $62.42_{\pm{0.28}}$& $18.06_{\pm{0.21}}$& $21.28_{\pm{0.05}}$& $23.88_{\p
% m{0.21}}$& $20.43_{\pm{0.48}}$\\
%     ~&\textbf{ER+TRADES+Ours}& $19.26_{\pm{0.38}}$& $58.26_{\pm{0.87}}$& $8.26_{\pm{0.14}}$& $7.56_{\pm{0.15}}$& $36.67_{\pm{0.14}}$& $63.45_{\pm{0.21}}$& $11.32_{\pm{0.41}}$& $31.66_{\pm{0.21}}$& $33.51_{\pm{0.30}}$& $14.26_{\pm{0.41}}$  \\
%     \bottomrule
%     \end{tabular}}
% \end{table*}






% \begin{table*}[]
%     \caption{The}
%     \label{Main-CIFAR100}
%     \centering % 居中显示
%     \scalebox{0.6}{
%     \begin{tabular}{lllllllllllll}
%     \toprule
%     \multirow{3}{*}{\textbf{Dataset}} &
%     \multirow{3}{*}{\textbf{Buffer Size}} &
%     \multirow{3}{*}{\textbf{Methods}} &
%     \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
%     ~&~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
%     ~&~&~&\textbf{FAA }&\textbf{Forgetting}&
%     \textbf{PGD-20}&
%     \textbf{AA}&
%     \textbf{Forgetting}&
%     \textbf{FAA }&\textbf{Forgetting}&
%     \textbf{PGD-20 }&
%     \textbf{AA}&
%     \textbf{Forgetting}\\
%     \midrule
%     \multirow{12}{*}{\textbf{Split-CIFAR10}}&\multirow{6}{*}{\textbf{200}}&\textbf{ER+AT}& $28.18_{\pm{0.69}}$ & $80.58_{\pm{1.05}}$ & $17.86_{\pm{0.29}}$ &$16.94_{\pm{0.38}}$ & $69.58_{\pm{1.15}}$ & $84.49_{\pm{0.61}}$ & $10.23_{\pm{0.98}}$ & $44.30_{\pm{1.05}}$ & $44.69_{\pm{1.04}}$ & $36.89_{\pm{1.11}}$  \\
%     ~&~&\textbf{ER+TRADES}& $22.42_{\pm{7.11}}$& $77.25_{\pm{10.79}}$& $15.72_{\pm{0.82}}$& $0_{\pm{0}}$& $64.95_{\pm{5.58}}$& $78.79_{\pm{0.81}}$& $8.1_{\pm{0.97}}$& $51.33_{\pm{2.3}}$& $0_{\pm{0}}$& $21.97_{\pm{1
% .31}}$  \\
%     ~&~&\textbf{ER+FAT}&$33.61_{\pm{6.80}}$ & $69.21_{\pm{8.95}}$ & $15.14_{\pm{0.80}}$ & 0 & $49.04_{\pm{7.29}) $& $83.40_{\pm{0.92}}$ & $10.35_{\pm{0.83}}$ & $43.69_{\pm{2.08}}$ & 0 & $28.56_{\pm{2.14}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \cmidrule(r){2-13}
%     ~&\multirow{6}{*}{\textbf{5120}}&\textbf{ER+AT} & $61.88_{\pm{0.74}}$ & $37.72_{\pm{0.73}}$ & $31.27_{\pm{0.63}}$ & $26.69_{\pm{0.52}}$ & $41.66_{\pm{1.22}}$ & $91.24_{\pm{0.19}}$ & $2.56_{\pm{0.12}}$ & $56.59_{\pm{0.88}}$ & $56.90_{\pm{0.88}}$ & $19.34_{\pm{1.11}}$\\
%     ~&~&\textbf{ER+TRADES}& $20.36_{\pm{2.81}}$& $85.14_{\pm{4.28}}$& $16.3_{\pm{0.44}}$& $0_{\pm{0}}$& $72.85_{\pm{1.46}}$& $88.48_{\pm{0.81}}$& $1.59_{\pm{0.86}}$& $64.36_{\pm{0.51}}$& $0_{\pm{0}}$& $12.47_{\pm{0
% .37}}$   \\
%     ~&~&\textbf{ER+FAT}& $54.55_{\pm{6.71}}$& $43.18_{\pm{7.51}}$& $19.68_{\pm{2.54}}$& $0_{\pm{0}}$& $42.15_{\pm{3.59}}$& $91.5_{\pm{0.53}}$& $2.12_{\pm{0.8}}$& $56.72_{\pm{0.65}}$& $0_{\pm{0}}$& $14.79_{\pm{1.
% 13}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \midrule
%     \multirow{12}{*}{\textbf{Split-CIFAR100}}&\multirow{6}{*}{\textbf{500}}&\textbf{ER+AT}&$11.72_{\pm{0.44}}$ & $74.22_{\pm{0.36}}$ & $6.01_{\pm{0.23}}$ & 0 & $37.47_{\pm{0.44}}$ & $54.53_{\pm{1.03}}$& $26.84_{\pm{0.88}}$ & $18.36_{\pm{0.43}}$ & 0 & $24.42_{\pm{0.74}}$  \\
%     ~&~&\textbf{ER+TRADES}& $7.59_{\pm{0.08}}$& $68.13_{\pm{0.61}}$& $5.43_{\pm{0.05}}$& $0_{\pm{0}}$& $44.13_{\pm{0.89}}$& $50.75_{\pm{0.42}}$& $20.22_{\pm{0.49}}$& $26.89_{\pm{0.58}}$& $0_{\pm{0}}$& $20.34_{\pm{0
% .72}}$   \\
%     ~&~&\textbf{ER+FAT}& $11.48_{\pm{0.72}}$& $73.99_{\pm{1.18}}$& $5.35_{\pm{0.26}}$& $0_{\pm{0}}$& $37.26_{\pm{0.62}}$& $56.1_{\pm{1.23}}$& $24.71_{\pm{1.0}}$& $20.01_{\pm{0.85}}$& $0_{\pm{0}}$& $22.31_{\pm{1.
% 1}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \cmidrule(r){2-13}
%     ~&\multirow{6}{*}{\textbf{2000}}&\textbf{ER+AT}& $15.45_{\pm{1.18}}$& $70.15_{\pm{1.24}}$& $6.08_{\pm{0.04}}$& $0_{\pm{0}}$& $36.35_{\pm{0.27}}$& $64.25_{\pm{0.15}}$& $16.34_{\pm{0.16}}$& $22.77_{\pm{0.68}}$& $0_{\pm{0}}$& $19.0_{\pm{0
% .59}}$  \\
%     ~&~&\textbf{ER+TRADES}& $9.5_{\pm{0.24}}$& $70.49_{\pm{0.38}}$& $5.35_{\pm{0.19}}$& $0_{\pm{0}}$& $42.08_{\pm{0.4}}$& $60.63_{\pm{1.03}}$& $13.78_{\pm{0.9}}$& $26.68_{\pm{0.51}}$& $0_{\pm{0}}$& $18.6_{\pm{0.54}
% }$   \\
%     ~&~&\textbf{ER+FAT}& $17.09_{\pm{1.96}}$& $66.91_{\pm{3.02}}$& $6.12_{\pm{0.4}}$& $0_{\pm{0}}$& $33.62_{\pm{1.72}}$& $63.88_{\pm{0.02}}$& $15.99_{\pm{0.47}}$& $23.48_{\pm{0.06}}$& $0_{\pm{0}}$& $17.12_{\pm{0
% .62}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
% \bottomrule
% \end{tabular}}
% \end{table*}

==> Tables/Pang_Results.tex <==
\begin{table*}[]
\begin{minipage}{\linewidth}
    \centering
    \centering % 居中显示
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llllllllllll}
    \toprule
    \multirow{3}{*}{\textbf{Buffer Size}} &
    \multirow{3}{*}{\textbf{Methods}} &
    \multicolumn{4}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{4}{c}{\textbf{Task Incremental Setting}} \\
    ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
    ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}\\
    \midrule
    {\textbf{200}}&\textbf{ER+Pang~\etal~\cite{pang2022robustness}}& $48.65_{\pm{1.76}}$& $56.79_{\pm{1.78}}$& $2.40_{\pm{0.46}}$& $0.93_{\pm{0.03}}$& $18.96_{\pm{2.47}}$& $88.90_{\pm{2.02}}$& $9.82_{\pm{2.53}}$& $7.25_{\pm{1.06}}$& $6.72_{\pm{0.55}}$& $8.70_{\pm{0.06}}$ \\
    {\textbf{5120}}&\textbf{ER+Pang~\etal~\cite{pang2022robustness}}& $51.37_{\pm{6.44}}$& $52.84_{\pm{8.47}}$& $3.14_{\pm{0.49}}$&$1.10_{\pm{0.05}}$& $20.29_{\pm{2.92}}$& $95.63_{\pm{0.17}}$& $1.58_{\pm{0.21}}$& $14.66_{\pm{0.15}}$&$13.92_{\pm{0.04}}$& $2.53_{\pm{0.46}}$\\
\bottomrule
\end{tabular}}
\subcaption{Results on Split-CIFAR10. We chose two buffer sizes of $200$ and $5120$.}
    \label{Pang-CIFAR10}
\end{minipage}

\begin{minipage}{\linewidth}
    \centering % 居中显示
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llllllllllll}
    \toprule
    \multirow{3}{*}{\textbf{Buffer Size}} &
    \multirow{3}{*}{\textbf{Methods}} &
    \multicolumn{4}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{4}{c}{\textbf{Task Incremental Setting}} \\
    ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
    ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}\\
    \midrule
    {\textbf{500}}&\textbf{ER+Pang~\etal~\cite{pang2022robustness}}& $16.22_{\pm{0.63}}$& $77.71_{\pm{0.44}}$& $0.91_{\pm{0.05}}$& $0.62_{\pm{0.00}}$& $6.13_{\pm{0.16}}$& $68.87_{\pm{0.25}}$& $11.21_{\pm{0.73}}$& $3.23_{\pm{0.42}}$& $7.95_{\pm{0.06}}$& $4.94_{\pm{0.05}}$\\
{\textbf{2000}}&\textbf{ER+Pang~\etal~\cite{pang2022robustness}}& $30.10_{\pm{0.53}}$& $61.51_{\pm{1.00}}$& $0.75_{\pm{0.22}}$&$0.51_{\pm{0.02}}$& $4.10_{\pm{0.60}}$& $76.90_{\pm{0.44}}$& $19.60_{\pm{0.32}}$& $4.88_{\pm{0.24}}$&$11.97_{\pm{0.26}}$& $5.25_{\pm{0.20}}$\\
    \bottomrule
    \end{tabular}}
    \subcaption{Results on Split-CIFAR100. We choose two buffer sizes of $500$ and $2000$.}
    \label{Pang-CIFAR100}
\end{minipage}


 \caption{Experiment results on Split-CIFAR10/100 dataset and model architecture is ResNet18.
    Here PGD-20 and are adversarial data Final Average Accuracy (FAA) generated by PGD-20. Forgetting of adversarial data is computed based on PGD-20.}
\label{PangCIFAR}
\end{table*}




% \begin{table*}[]
%     \caption{Experiment results on Split-CIFAR100 dataset and model architecture is ResNet18.
%     Following~\cite{buzzega2020dark}, we choose two buffer sizes of 500 and 2000.
%     Here PGD-20 and AA are adversarial data Final Average Accuracy (FAA) generated by PGD-20 and Auto Attack (AA) respectively. Forgetting of adversarial data is computed based on PGD-20.}
%     \label{Main-CIFAR100}
%     \centering % 居中显示
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{llllllllllll}
%     \toprule
%     \multirow{3}{*}{\textbf{Buffer Size}} &
%     \multirow{3}{*}{\textbf{Methods}} &
%     \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
%     ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
%     ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{AA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{FAA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}&
%     \textbf{PGD-20$\uparrow$}&
%     \textbf{AA$\uparrow$}&
%     \textbf{Forgetting$\downarrow$}\\
%     \midrule
%     \multirow{6}{*}{\textbf{500}}&\textbf{ER+AT}& $11.94_{\pm{0.74}}$& $73.54_{\pm{0.75}}$& $5.66_{\pm{0.31}}$& $5.54_{\pm{0.31}}$& $38.03_{\pm{0.1}}$& $52.71_{\pm{0.96}}$& $28.44_{\pm{1.11}}$& $17.35_{\pm{0.08}}$& $19.56_{\pm
% {0.1}}$& $25.67_{\pm{0.26}}$  \\
%     ~&\textbf{ER+TRADES}& $7.59_{\pm{0.08}}$& $68.13_{\pm{0.61}}$& $5.43_{\pm{0.05}}$& $5.11_{\pm{0.06}}$& $44.13_{\pm{0.89}}$& $50.75_{\pm{0.42}}$& $20.22_{\pm{0.49}}$& $26.89_{\pm{0.58}}$& $27.69_{\pm{0.56}}$& $20.34_{\pm{0
% .72}}$   \\
%     ~&\textbf{ER+FAT}& $11.48_{\pm{0.72}}$& $73.99_{\pm{1.18}}$& $5.35_{\pm{0.26}}$& $5.23_{\pm{0.27}}$& $37.26_{\pm{0.62}}$& $56.1_{\pm{1.23}}$& $24.71_{\pm{1.00}}$& $20.01_{\pm{0.85}}$& $22.99_{\pm{0.91}}$& $22.31_{\pm{1.10}}$  \\
%     ~&\textbf{ER+LBGAT}& $11.77_{\pm{0.37}}$& $75.1_{\pm{0.4}}$& $6.16_{\pm{0.11}}$& $5.82_{\pm{0.13}}$& $39.77_{\pm{0.18}}$& $42.02_{\pm{2.36}}$& $26.45_{\pm{0.3}}$& $13.99_{\pm{0.83}}$& $14.43_{\pm{0.97}}$& $23.14_{\pm{0.21}}$ \\
%     \cmidrule(r){2-12}
%     ~&\textbf{ER+AT+Ours}& $17.5_{\pm{0.39}}$& $66.66_{\pm{0.11}}$& $6.76_{\pm{0.36}}$& $6.49_{\pm{0.34}}$& $34.54_{\pm{0.24}}$& $53.1_{\pm{1.46}}$& $28.59_{\pm{1.51}}$& $17.34_{\pm{0.41}}$& $19.04_{\pm{
% 0.56}}$& $25.77_{\pm{0.66}}$ \\
%     ~&\textbf{ER+TRADES+Ours}& $14.61_{\pm{1.15}}$& $62.63_{\pm{2.25}}$& $7.15_{\pm{0.22}}$& $6.42_{\pm{0.23}}$& $37.49_{\pm{2.31}}$& $54.65_{\pm{0.94}}$& $20.56_{\pm{0.51}}$& $27.72_{\pm{0.94}}$& $28.50_{\pm{0.55}}$& $18.25_{\pm{1.28}}$  \\
%     \cmidrule(r){1-12}
%     \multirow{6}{*}{\textbf{2000}}&\textbf{ER+AT}& $18.77_{\pm{0.18}}$& $65.06_{\pm{0.58}}$& $7.2_{\pm{0.18}}$& $7.01_{\pm{0.18}}$& $33.56_{\pm{0.26}}$& $62.01_{\pm{0.76}}$& $17.97_{\pm{0.8}}$& $21.16_{\pm{0.38}}$& $24.04_{\pm{
% 0.23}}$& $20.47_{\pm{0.25}}$ \\
%     ~&\textbf{ER+TRADES}& $9.50_{\pm{0.24}}$& $70.49_{\pm{0.38}}$& $5.35_{\pm{0.19}}$& $5.01_{\pm{0.17}}$& $42.08_{\pm{0.4}}$& $60.63_{\pm{1.03}}$& $13.78_{\pm{0.9}}$& $26.68_{\pm{0.51}}$& $29.19_{\pm{0.70}}$& $18.6_{\pm{0.54}
% }$   \\
%     ~&\textbf{ER+FAT}& $17.09_{\pm{1.96}}$& $66.91_{\pm{3.02}}$& $6.12_{\pm{0.4}}$& $5.93_{\pm{0.38}}$& $33.62_{\pm{1.72}}$& $63.88_{\pm{0.02}}$& $15.99_{\pm{0.47}}$& $23.48_{\pm{0.06}}$& $26.75_{\pm{0.05}}$& $17.12_{\pm{0.62}}$  \\
%     ~&\textbf{ER+LBGAT}& $20.58_{\pm{0.15}}$& $63.31_{\pm{0.2}}$& $7.93_{\pm{0.17}}$& $0.0_{\pm{0.0}}$& $30.09_{\pm{0.32}}$& $55.77_{\pm{0.23}}$& $25.11_{\pm{0.54}}$& $17.95_{\pm{0.43}}$& $0.0_{\pm{0.0
% }}$& $19.18_{\pm{0.48}}$\\
%     \cmidrule(r){2-12}
%     ~&\textbf{ER+AT+Ours}& $24.52_{\pm{0.37}}$& $57.28_{\pm{0.34}}$& $8.58_{\pm{0.24}}$& $8.25_{\pm{0.25}}$& $28.44_{\pm{0.18}}$& $62.42_{\pm{0.28}}$& $18.06_{\pm{0.21}}$& $21.28_{\pm{0.05}}$& $23.88_{\p
% m{0.21}}$& $20.43_{\pm{0.48}}$\\
%     ~&\textbf{ER+TRADES+Ours}& $19.26_{\pm{0.38}}$& $58.26_{\pm{0.87}}$& $8.26_{\pm{0.14}}$& $7.56_{\pm{0.15}}$& $36.67_{\pm{0.14}}$& $63.45_{\pm{0.21}}$& $11.32_{\pm{0.41}}$& $31.66_{\pm{0.21}}$& $33.51_{\pm{0.30}}$& $14.26_{\pm{0.41}}$  \\
%     \bottomrule
%     \end{tabular}}
% \end{table*}






% \begin{table*}[]
%     \caption{The}
%     \label{Main-CIFAR100}
%     \centering % 居中显示
%     \scalebox{0.6}{
%     \begin{tabular}{lllllllllllll}
%     \toprule
%     \multirow{3}{*}{\textbf{Dataset}} &
%     \multirow{3}{*}{\textbf{Buffer Size}} &
%     \multirow{3}{*}{\textbf{Methods}} &
%     \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
%     ~&~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}&
%     \multicolumn{2}{c}{\textbf{Clean Data}}&
%     \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
%     ~&~&~&\textbf{FAA }&\textbf{Forgetting}&
%     \textbf{PGD-20}&
%     \textbf{AA}&
%     \textbf{Forgetting}&
%     \textbf{FAA }&\textbf{Forgetting}&
%     \textbf{PGD-20 }&
%     \textbf{AA}&
%     \textbf{Forgetting}\\
%     \midrule
%     \multirow{12}{*}{\textbf{Split-CIFAR10}}&\multirow{6}{*}{\textbf{200}}&\textbf{ER+AT}& $28.18_{\pm{0.69}}$ & $80.58_{\pm{1.05}}$ & $17.86_{\pm{0.29}}$ &$16.94_{\pm{0.38}}$ & $69.58_{\pm{1.15}}$ & $84.49_{\pm{0.61}}$ & $10.23_{\pm{0.98}}$ & $44.30_{\pm{1.05}}$ & $44.69_{\pm{1.04}}$ & $36.89_{\pm{1.11}}$  \\
%     ~&~&\textbf{ER+TRADES}& $22.42_{\pm{7.11}}$& $77.25_{\pm{10.79}}$& $15.72_{\pm{0.82}}$& $0_{\pm{0}}$& $64.95_{\pm{5.58}}$& $78.79_{\pm{0.81}}$& $8.1_{\pm{0.97}}$& $51.33_{\pm{2.3}}$& $0_{\pm{0}}$& $21.97_{\pm{1
% .31}}$  \\
%     ~&~&\textbf{ER+FAT}&$33.61_{\pm{6.80}}$ & $69.21_{\pm{8.95}}$ & $15.14_{\pm{0.80}}$ & 0 & $49.04_{\pm{7.29}) $& $83.40_{\pm{0.92}}$ & $10.35_{\pm{0.83}}$ & $43.69_{\pm{2.08}}$ & 0 & $28.56_{\pm{2.14}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \cmidrule(r){2-13}
%     ~&\multirow{6}{*}{\textbf{5120}}&\textbf{ER+AT} & $61.88_{\pm{0.74}}$ & $37.72_{\pm{0.73}}$ & $31.27_{\pm{0.63}}$ & $26.69_{\pm{0.52}}$ & $41.66_{\pm{1.22}}$ & $91.24_{\pm{0.19}}$ & $2.56_{\pm{0.12}}$ & $56.59_{\pm{0.88}}$ & $56.90_{\pm{0.88}}$ & $19.34_{\pm{1.11}}$\\
%     ~&~&\textbf{ER+TRADES}& $20.36_{\pm{2.81}}$& $85.14_{\pm{4.28}}$& $16.3_{\pm{0.44}}$& $0_{\pm{0}}$& $72.85_{\pm{1.46}}$& $88.48_{\pm{0.81}}$& $1.59_{\pm{0.86}}$& $64.36_{\pm{0.51}}$& $0_{\pm{0}}$& $12.47_{\pm{0
% .37}}$   \\
%     ~&~&\textbf{ER+FAT}& $54.55_{\pm{6.71}}$& $43.18_{\pm{7.51}}$& $19.68_{\pm{2.54}}$& $0_{\pm{0}}$& $42.15_{\pm{3.59}}$& $91.5_{\pm{0.53}}$& $2.12_{\pm{0.8}}$& $56.72_{\pm{0.65}}$& $0_{\pm{0}}$& $14.79_{\pm{1.
% 13}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \midrule
%     \multirow{12}{*}{\textbf{Split-CIFAR100}}&\multirow{6}{*}{\textbf{500}}&\textbf{ER+AT}&$11.72_{\pm{0.44}}$ & $74.22_{\pm{0.36}}$ & $6.01_{\pm{0.23}}$ & 0 & $37.47_{\pm{0.44}}$ & $54.53_{\pm{1.03}}$& $26.84_{\pm{0.88}}$ & $18.36_{\pm{0.43}}$ & 0 & $24.42_{\pm{0.74}}$  \\
%     ~&~&\textbf{ER+TRADES}& $7.59_{\pm{0.08}}$& $68.13_{\pm{0.61}}$& $5.43_{\pm{0.05}}$& $0_{\pm{0}}$& $44.13_{\pm{0.89}}$& $50.75_{\pm{0.42}}$& $20.22_{\pm{0.49}}$& $26.89_{\pm{0.58}}$& $0_{\pm{0}}$& $20.34_{\pm{0
% .72}}$   \\
%     ~&~&\textbf{ER+FAT}& $11.48_{\pm{0.72}}$& $73.99_{\pm{1.18}}$& $5.35_{\pm{0.26}}$& $0_{\pm{0}}$& $37.26_{\pm{0.62}}$& $56.1_{\pm{1.23}}$& $24.71_{\pm{1.0}}$& $20.01_{\pm{0.85}}$& $0_{\pm{0}}$& $22.31_{\pm{1.
% 1}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
%     \cmidrule(r){2-13}
%     ~&\multirow{6}{*}{\textbf{2000}}&\textbf{ER+AT}& $15.45_{\pm{1.18}}$& $70.15_{\pm{1.24}}$& $6.08_{\pm{0.04}}$& $0_{\pm{0}}$& $36.35_{\pm{0.27}}$& $64.25_{\pm{0.15}}$& $16.34_{\pm{0.16}}$& $22.77_{\pm{0.68}}$& $0_{\pm{0}}$& $19.0_{\pm{0
% .59}}$  \\
%     ~&~&\textbf{ER+TRADES}& $9.5_{\pm{0.24}}$& $70.49_{\pm{0.38}}$& $5.35_{\pm{0.19}}$& $0_{\pm{0}}$& $42.08_{\pm{0.4}}$& $60.63_{\pm{1.03}}$& $13.78_{\pm{0.9}}$& $26.68_{\pm{0.51}}$& $0_{\pm{0}}$& $18.6_{\pm{0.54}
% }$   \\
%     ~&~&\textbf{ER+FAT}& $17.09_{\pm{1.96}}$& $66.91_{\pm{3.02}}$& $6.12_{\pm{0.4}}$& $0_{\pm{0}}$& $33.62_{\pm{1.72}}$& $63.88_{\pm{0.02}}$& $15.99_{\pm{0.47}}$& $23.48_{\pm{0.06}}$& $0_{\pm{0}}$& $17.12_{\pm{0
% .62}}$  \\
%     ~&~&\textbf{ER+LBGAT}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     \cmidrule(r){3-13}
%     ~&~&\textbf{ER+AT+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0 \\
%     ~&~&\textbf{ER+TRADES+Ours}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0 & 0 & 0  \\
% \bottomrule
% \end{tabular}}
% \end{table*}

==> Tables/TinyImageNet_std.tex <==
\begin{table*}[]
    \centering % 居中显示
     \caption{Experiment results on S-Tiny-ImageNet dataset and model architecture is ResNet18.
    Following~\cite{buzzega2020dark}, we choose two buffer sizes of 200 and 5120.
    Here PGD-20 and AA are adversarial data Final Average Accuracy (FAA) generated by PGD-20 and Auto Attack (AA) respectively. Forgetting of adversarial data is computed based on PGD-20. \textbf{Bold} represents the best experimental results for the same settings. With the addition of ours, model performance can be improved across the board.}
    \label{Main-TinyImg_std}
    \resizebox{\textwidth}{!}{

    \begin{tabular}{llllllllllll}
    \toprule
    \multirow{3}{*}{\textbf{Buffer Size}} &
    \multirow{3}{*}{\textbf{Methods}} &
    \multicolumn{5}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{5}{c}{\textbf{Task Incremental Setting}} \\
    ~&~&\multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}&
    \multicolumn{2}{c}{\textbf{Clean Data}}&
    \multicolumn{3}{c}{\textbf{Adversarial Data}}\\
    ~&~&\textbf{FAA$\uparrow$ }&\textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{FAA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}&
    \textbf{PGD-20$\uparrow$}&
    \textbf{AA$\uparrow$}&
    \textbf{Forgetting$\downarrow$}\\
    \midrule
    \multirow{2}{*}{\textbf{200}}&\textbf{ER+TRADES} & $5.50_{\pm{0.41}}$ & $54.67_{\pm{0.13}}$ & $2.04_{\pm{0.35}}$ & $1.92_{\pm{0.35}}$ & $22.62_{\pm{0.21}}$ & $23.51_{\pm{1.38}}$ & $34.72_{\pm{1.15}}$ & $5.28_{\pm{0.73}}$ & $6.48_{\pm{0.91}}$ & $19.10_{\pm{0.42}}$    \\
    ~&\textbf{ER+TRADES+Ours}&\pmb{$7.35_{\pm{0.43}}$} &\pmb{$52.38_{\pm{0.22}}$} &\pmb{$2.22_{\pm{0.08}}$} &\pmb{$2.05_{\pm{0.03}}$} &\pmb{$20.79_{\pm{0.14}}$} &\pmb{$25.58_{\pm{0.73}}$} &\pmb{$34.94_{\pm{1.44}}$} &\pmb{$6.24_{\pm{0.30}}$} &\pmb{$7.60_{\pm{0.26}}$} &\pmb{$18.41_{\pm{0.20}}$}  \\
    \cmidrule(r){1-12}
    \multirow{2}{*}{\textbf{5120}}&\textbf{ER+TRADES}& $7.24_{\pm{0.39}}$ & $55.69_{\pm{1.06}}$ & $2.39_{\pm{0.16}}$ & $2.21_{\pm{0.14}}$ & $21.59_{\pm{0.91}}$ & $41.36_{\pm{1.07}}$ & $18.16_{\pm{1.74}}$ & $11.01_{\pm{0.92}}$ & $13.71_{\pm{0.78}}$ & $12.61_{\pm{1.45}}$ \\
    ~&\textbf{ER+TRADES+Ours}&\pmb{$10.95_{\pm{0.8}}$} &\pmb{$51.63_{\pm{1.11}}$} &\pmb{$3.01_{\pm{0.24}}$} &\pmb{$2.79_{\pm{0.25}}$} &\pmb{$21.74_{\pm{0.6}}$} &\pmb{$44.81_{\pm{0.13}}$} &\pmb{$15.20_{\pm{0.08}}$} &\pmb{$12.92_{\pm{0.16}}$} &\pmb{$16.21_{\pm{0.06}}$} &\pmb{$12.33_{\pm{0.42}}$}\\
    \bottomrule
    % \midrule
    \end{tabular}
    }
\end{table*}

==> Tables/adaptive_attack_std.tex <==
\begin{table*}[]
 \caption{Adaptive Attack for ER+TRADES+ours. All the attack methods in the table incorporate the same logit calibration as in the training phase of our model. Forgetting is based on PGD-20. Results show our method still maintains decent robustness.}
    \label{adaptive_std}
    \centering % 居中显示
    \scalebox{1.15}{
    \begin{tabular}{ll lll lll}
    \toprule
    \multirow{2}{*}{\textbf{Dataset}} &
    \multirow{1}{*}{\textbf{Buffer}}&
    \multicolumn{3}{c}{\textbf{Class Incremental Setting}} &
    \multicolumn{3}{c}{\textbf{Task Incremental Setting}} \\
    ~&\multirow{1}{*}{\textbf{Size}}&\textbf{ PGD-20 }&
    \textbf{ AA}&
    \textbf{Forgetting}&
    \textbf{ PGD-20 }&
    \textbf{AA}&
    \textbf{Forgetting}\\
    \midrule
    \multirow{2}{*}{\textbf{CIFAR-10}}&\textbf{200}&
    $23.99_{\pm{1.36}}$&$41.76_{\pm{0.00}}$&$26.43_{\pm{8.04}}$&$58.18_{\pm{0.17}}$&$58.32_{\pm{0.26}}$&$15.40_{\pm{0.26}}$\\
    % $23.13_{\pm{1.87}}$ & $41.39_{\pm{4.58}}$ & $38.35_{\pm{8.56}}$& $59.41_{\pm{0.63}}$ &$59.60_{\pm{0.63}}$& $14.16_{\pm{1.28}}$ \\
    ~&\textbf{5120}&
    $27.50_{\pm{2.80}}$&$35.29_{\pm{0.52}}$&$1.53_{\pm{0.69}}$&$65.59_{\pm{3.26}}$&$60.69_{\pm{0.50}}$&$5.89_{\pm{3.20}}$\\
    % $23.62_{\pm{6.77}}$ & $37.22_{\pm{12.19}}$ & $41.96_{\pm{12.00}}$ & $69.27_{\pm{2.23}}$ & $69.35_{\pm{2.24}}$& $5.31_{\pm{0.75}}$\\
    \midrule
    \multirow{2}{*}{\textbf{CIFAR-100}}&\textbf{500}&
    $9.91_{\pm{0.52}}$&$20.61_{\pm{0.98}}$&$13.10_{\pm{1.52}}$&$26.84_{\pm{0.94}}$&$28.20_{\pm{0.72}}$&$17.13_{\pm{0.79}}$\\
    % $7.40_{\pm{0.54}}$ & $11.83_{\pm{1.22}}$ & $38.78_{\pm{1.37}}$ & $27.64_{\pm{0.96}}$ & $28.84_{\pm{0.56}}$ & $18.13_{\pm{1.28}}$\\
    ~&\textbf{2000}&
    $13.68_{\pm{0.93}}$&$25.85_{\pm{0.73}}$&$15.33_{\pm{1.02}}$&$34.83_{\pm{0.62}}$&$35.72_{\pm{0.84}}$&$11.59_{\pm{0.42}}$\\
    % $8.68_{\pm{0.20}}$ & $16.15_{\pm{0.38}}$ & $37.87_{\pm{0.08}}$ & $31.48_{\pm{0.18}}$ & $33.83_{\pm{0.28}}$& $14.21_{\pm{0.34}}$\\
\bottomrule
\end{tabular}}
   
\end{table*}


% \begin{table*}[]
%     \caption{Adaptive Attack for ours}
%     \label{adaptive}
%     \centering % 居中显示
%     \scalebox{0.7}{
%     \begin{tabular}{lllllllllll}
%     \toprule
%     \multirow{2}{*}{\textbf{Dataset}} &
%     \multirow{2}{*}{\textbf{Buffer Size}}&
%     \multirow{2}{*}{\textbf{Baseline}} &
%     \multicolumn{4}{c}{\textbf{Class Incremental Setting}} &
%     \multicolumn{4}{c}{\textbf{Task Incremental Setting}} \\
%     ~&~&~&\textbf{ PGD-20 }&
%     \textbf{ AA}&
%     \textbf{ PGD-20 Forgetting}&
%     \textbf{ AA Forgetting}&
%     \textbf{ PGD-20 }&
%     \textbf{AA}&
%     \textbf{PGD-20 Forgetting}&
%     \textbf{AA Forgetting}\\
%     \midrule
%     \multirow{4}{*}{\textbf{CIFAR-10}}&\multirow{2}{*}{\textbf{200}}&
%     \textbf{AT}&0 & 0 & 0 & 0& 0 & 0& 0 & 0 \\
%     ~&~&\textbf{TRADES}&$23.13_{\pm{1.87}}$ & 0 & $38.35_{\pm{8.56}}$ & 0 & $59.41_{\pm{0.63}}$ & 0& $14.16_{\pm{1.28}}$ & 0\\
%     ~&\multirow{2}{*}{\textbf{5120}}&
%     \textbf{AT}&0 & 0 & 0 & 0& 0 & 0& 0 & 0 \\
%     ~&~&\textbf{TRADES}&$23.62_{\pm{6.77}}$ & 0 & $41.96_{\pm{12.00}}$ & 0 & $69.27_{\pm{2.23}}$ & 0& $5.31_{\pm{0.75}}$& 0\\
%     \midrule
%     \multirow{4}{*}{\textbf{CIFAR-100}}&\multirow{2}{*}{\textbf{500}}&
%     \textbf{AT}&0 & 0 & 0 & 0& 0 & 0& 0 & 0 \\
%     ~&~&\textbf{TRADES}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0\\
%     ~&\multirow{2}{*}{\textbf{2000}}&
%     \textbf{AT}&0 & 0 & 0 & 0& 0 & 0& 0 & 0 \\
%     ~&~&\textbf{TRADES}&0 & 0 & 0 & 0 & 0 & 0& 0 & 0\\
% \bottomrule
% \end{tabular}}
% \end{table*}

==> macros.tex <==
\usepackage{ifthen}
\usepackage{xcolor}


\definecolor{YongColor}{rgb}{0.0,0.1,0.9}
\definecolor{FanColor}{rgb}{0.8,0,0.8}
\definecolor{XiaoyueColor}{rgb}{0,0.6,0.6}


\newcommand{\increase}[1]{{\color{teal}(+#1)}}
\newcommand{\decrease}[1]{{\color{red}(-#1)}}

\newcommand{\yong}[1]{{\color{YongColor}[Yong: #1]}}

\newcommand{\fan}[1]{{\color{FanColor}[Fan: #1]}}

\newcommand{\xiaoyue}[1]{{\color{XiaoyueColor}[xiaoyue: #1]}}

\newcommand{\warning}[1]{{\it\color{red} #1}}
\newcommand{\toremove}[1]{{\it\color{red} (To remove) #1}}
\newcommand{\nothing}[1]{}

\ifthenelse{\equal{\final}{1}}
{

\renewcommand{\fan}[1]{}
\renewcommand{\yong}[1]{}
\renewcommand{\xiaoyue}[1]{}

\renewcommand{\warning}[1]{}
\renewcommand{\toremove}[1]{}
\renewcommand{\nothing}[1]{}
}{}

\hyphenpenalty=1000 % magic number to reduce ugly line breaks

\newcommand{\inputsection}[1]{\input{Sections/#1}}
\newcommand{\inputfigure}[1]{\input{Figures/#1}}
\newcommand{\inputtable}[1]{\input{Tables/#1}}
\newcommand{\citep}[1]{\cite#1}
%\newcommand{\etal}[0]{~et al.}
\newcommand{\figtext}[1]{{\footnotesize #1}}
